Collective Graph Exploration Parameterized by Vertex Cover

We initiate the study of the parameterized complexity of the {\sc Collective Graph Exploration} ({\sc CGE}) problem. In {\sc CGE}, the input consists of an undirected connected graph $G$ and a collection of $k$ robots, initially placed at the same vertex $r$ of $G$, and each one of them has an energy budget of $B$. The objective is to decide whether $G$ can be \emph{explored} by the $k$ robots in $B$ time steps, i.e., there exist $k$ closed walks in $G$, one corresponding to each robot, such that every edge is covered by at least one walk, every walk starts and ends at the vertex $r$, and the maximum length of any walk is at most $B$. Unfortunately, this problem is \textsf{NP}-hard even on trees [Fraigniaud {\em et~al.}, 2006]. Further, we prove that the problem remains \textsf{W[1]}-hard parameterized by $k$ even for trees of treedepth $3$. Due to the \textsf{para-NP}-hardness of the problem parameterized by treedepth, and motivated by real-world scenarios, we study the parameterized complexity of the problem parameterized by the vertex cover number ($\mathsf{vc}$) of the graph, and prove that the problem is fixed-parameter tractable (\textsf{FPT}) parameterized by $\mathsf{vc}$. Additionally, we study the optimization version of {\sc CGE}, where we want to optimize $B$, and design an approximation algorithm with an additive approximation factor of $O(\mathsf{vc})$.

==> Conclusion.tex <==
\section{Conclusion}\label{sec:conclusion}


==> Theorem.tex <==
%!TEX root =Main-Movement.tex

\section{The Decomposition}\label{sec:theorem}

Given a rectilinear graph $G=(V,E)$, our objective is to find a simple geometric decomposition of $G$. Specifically, we would like to ``split" the graph into columns-wise aligned rectangles with particular properties (described later). 
For a grid graph $G=(V,E)$, we denote the following:  

\begin{itemize}
\item $r_{\mathrm{min}}=\mathrm{min}\{ r\in \mathbb{N}_0~|~$there exists $c\in \mathbb{N}_0$ such that $(r,c)\in V \}$.
\item $c_{\mathrm{min}}=\mathrm{min}\{ c\in \mathbb{N}_0~|~$there exists $r\in \mathbb{N}_0$ such that $(r,c)\in V \}$.
\end{itemize}

Without loss of generality, we assume that $r_{\mathrm{min}}=c_{\mathrm{min}}=1$, otherwise we can modify $G$ as follows. For every vertex $u_{a,b}\in V$, we replace it by the vertex $u_{a - {r}_{\mathrm{min}}+1, b - {c}_{\mathrm{min}}+1 }$. Intuitively, this operation ``shifts'' the entire grid graph $G$ in parallel to the axes. 

We now define the notion of a {\em rectangle grid graph}, to be used throughout the paper.

%We begin by defining exactly what graph we split into rectangles. We want a graph which is in a ``shape" of a rectangle, and which is as ``small" as possible, such that it contains any connected grid graph $G=(V,E)$ with $|V|$ vertices. For that purpose, we have the following definitions. First we define a {\em rectangle grid graph}. A rectangle grid graph is a grid graph which has an ``outer shape" of a rectangle and ``contains" all the vertices inside it, as we define in the next definition.      


\begin{definition} [{\bf Rectangle Grid Graph}]\label{def:Rectangle grid graph}
A {\em rectangle grid graph} is a grid graph $G=(V,E)$ where, for every two vertices $u_{a_1,b_1},u_{a_2,b_2}\in V$, the following condition is satisfied: For every $a,b\in \mathbb{N}_0$ such that $a_{\min}\leq a\leq a_{\max}$ and $b_{\min}\leq b\leq b_{\max}$, where $a_{\min}=\min\{a_1,a_2\}$, $a_{\max}=\max\{a_1,a_2\}$, $b_{\min}=\min\{b_1,b_2\}$ and $b_{\max}=\max\{b_1,b_2\}$, it holds that $u_{a,b}\in V$.  
\end{definition}

For the sake of simplicity, sometimes we refer to rectangle grid graphs simply as rectangles.  

For our purposes, we would like to highlight two out of the four ``corners" of a rectangle grid graph: We denote the vertices in the top left and in the bottom right, respectively, by $u_{r_{min},c_{min}}, u_{r_{max},c_{max}}$, as it follows from the next observation.  

\begin{observation}  \label{obs:Rectangle grid graph is a matrix}
For a rectangle grid graph $G=(V,E)$, there exist unique $r_{min},r_{max},c_{min},c_{max}$ $\in \mathbb{N}_0$ such that $u_{r_{min},c_{min}}, u_{r_{max},c_{max}}\in V$, and for every $a,b\in \mathbb{N}_0$ such that $r_{max}<a$ or $a<r_{min}$ or $c_{max}<b$ or $b<c_{min}$, it holds that $u_{a,b}\notin V$. 

Moreover, for every $r_{min}\leq r_{max},c_{min}\leq c_{max}\in \mathbb{N}_0$, there exists a unique rectangle grid graph $G=(V,E)$ such that $u_{r_{min},c_{min}}, u_{r_{max},c_{max}}\in V$, and for every $a,b\in \mathbb{N}_0$ such that $r_{max}<a$ or $a<r_{min}$ or $c_{max}<b$ or $b<c_{min}$, it holds that $u_{a,b}\notin V$.     
\end{observation}



Let $G=(V,E)$ be a rectangle grid graph. We say that a vertex $u_{i,j}\in V$ is {\em located at the $i$-th row and $j$-th column}. Additionally, we say that $G$ has $r_{max}+1$ rows and $c_{max}+1$ columns.

We now define a {\em super rectangle grid graph} of a grid graph $G=(V,E)$.
%As we state before, we would like a rectangle grid graph that contains our given grid graph $G=(V,E)$. We call this kind of rectangle grid graph, a {\em super rectangle grid graph} of $G=(V,E)$, as we state in the next definition.   

\begin{definition}  [{\bf Super Rectangle Grid Graph}] \label{def:Super rectangle grid graph}
The {\em super rectangle grid graph} of a rectilinear graph $G=(V,E)$ is the grid graph $H=(V',E')$ where $V'= \{u_{i,j}~|~0\leq i\leq r_{max}+1,0\leq i\leq c_{max}+1\}$ and for every $u_{i,j},u_{i',j'}\in V'$,  $\{ u_{i,j},u_{i',j'}\}\in E'$ if and only if $|i-i'|+|j-j'|=1$.     
\end{definition}



Observe that the super rectangle grid graph of $G=(V,E)$, $H=(V',E')$, is a rectangle grid graph such that $V\subseteq V'$.
When $G$ is clear from the context, we refer to the super rectangle grid graph of $G=(V,E)$, $H=(V',E')$, simply as $H$. 


%We would like to get a ``general" super rectangle grid graph of $G=(V,E)$. For that purpose we define an {\em $H(|V|)$-graph}. An $H(|V|)$-graph is the rectangle grid graph that its top left vertex is $\{0,0\}$ and has $n+1$ column and rows, where $|V|=n$. It is easy to see that $H(|V|)$-graph is a super rectangle grid graph of $G$ as we state in Observation \ref{obs:rectsup}.    

%\begin{definition}  [{\bf Super Rectangle Grid Graph}] \label{def:Super rectangle grid graph}
%A {\em super rectangle grid graph} of a grid graph $G=(V,E)$ is a rectangle grid graph $H=(V',E')$ such that $V\subseteq V'$.     
%\end{definition}     

%\begin{definition}  [{\bf $H(|V|)$-graph}] \label{def:Super rectangle grid graph H}
%Let $G=(V,E)$ be a grid graph. Then {\em $H(|V|)$-graph} is the grid graph $H=(V',E')$ where $V'= \{\{i,j\}~|~0\leq i,j\leq |V|+1\}$ and for every $\{i,j\},\{i',j'\}\in V$  $\{ \{i,j\},\{i',j'\}\}\in E$ if and only if $|i-i'|+|j-j'|=1$.   
%\end{definition}

%\begin{definition}  [{\bf $H(|V|)$-graph}] \label{def:Super rectangle grid graph H}
%Let $G=(V,E)$ be a grid graph. Then {\em $H(|V|)$-graph} is the grid graph $H=(V',E')$ where $V'= \{\{i,j\}~|~0\leq i,j\leq |V|+1\}$ and for every $\{i,j\},\{i',j'\}\in V$  $\{ \{i,j\},\{i',j'\}\}\in E$ if and only if $|i-i'|+|j-j'|=1$.   
%\end{definition}


%\begin{observation}\label{obs:rectsup}
%Let $G=(V,E)$ be a connected grid graph. Then $H=(V',E')$ is a super rectangle grid graph of $G$.
%\end{observation}

%As $H$ is a rectangle grid graph and is easier to handle than $G$, our algorithm first computes a decomposition of $H$. Given a decomposition of $H$, we will easily compute the decomposition of $G$. 
 

%From that point forward, we would like to split the $H(|V|)$-graph into columns-lined-up rectangles. The algorithm we provide later in this paper indeed splits the $H(|V|)$-graph into columns-lined-up rectangles, but can easily adapt to split other super rectangle grid graphs of $G$.

% \begin{definition}  [{\bf L Shape Edge}] \label{def:LShapeEdge}
%Let $G=(V,E)$ be a rectilinear graph and let $H=(V',E')$ be the super rectangle grid graph} of a grid graph $G=(V,E)$ is the grid graph $H=(V',E')$ where $V'= \{u_{i,j}~|~0\leq i\leq r_{max}+1,0\leq i\leq c_{max}+1\}$ and for every $u_{i,j},u_{i',j'}\in V'$,  $\{ u_{i,j},u_{i',j'}\}\in E'$ if and only if $|i-i'|+|j-j'|=1$.     
%\end{definition}

\begin{definition}  [{\bf Drawn Separator}] \label{def:drawnSeparator}
Let $G=(V,E)$ be a rectilinear graph and let $H=(V',E')$ be the super rectangle grid graph of $G$. A {\em drawn separator} is a path in $H$, $(u_{a_0,b_0},\ldots,u_{a_\ell,b_\ell})$ such that the following conditions are satisfied:
\begin{enumerate}
\item $a_0=0$ or $a_0=r_{max}+1$ or $b_0=0$ or $b_0=c_{max}+1$.
\item $a_\ell=0$ or $a_\ell=r_{max}+1$ or $b_\ell=0$ or $b_\ell=c_{max}+1$. 
\item For every $0< i< \ell$, $a_i\neq 0$, $a_i\neq r_{max}+1$, $b_i\neq 0$, $b_i\neq c_{max}+1$.
\item For every $1\leq i< \ell-1$, $u_{a_i,b_i}\in V$ or $u_{a_{i+1},b_{i+1}}\in V$.    
\end{enumerate}      
\end{definition}



\begin{definition}  [{\bf Drawn Treewidth Decomposition}] \label{def:drawntreewisthDeco}
Let $G=(V,E)$ be a rectilinear graph and let $H=(V',E')$ be the super rectangle grid graph of $G$. A {\em drawn separator} is a path in $H$, $(u_{a_0,b_0},\ldots,u_{a_\ell,b_\ell})$ such that the following conditions are satisfied:
\begin{enumerate}
\item $a_0=0$ or $a_0=r_{max}+1$ or $b_0=0$ or $b_0=c_{max}+1$.
\item $a_\ell=0$ or $a_\ell=r_{max}+1$ or $b_\ell=0$ or $b_\ell=c_{max}+1$. 
\item For every $0< i< \ell$, $a_i\neq 0$, $a_i\neq r_{max}+1$, $b_i\neq 0$, $b_i\neq c_{max}+1$.
\item For every $1\leq i< \ell-1$, $u_{a_i,b_i}\in V$ or $u_{a_{i+1},b_{i+1}}\in V$.    
\end{enumerate}      
\end{definition}


\begin{observation}
Let $G=(V,E)$ be a rectilinear graph and let $H=(V',E')$ be the super rectangle grid graph of $G$. 

\end{observation}

Now, we define formally our decomposition. In what follows, we consider a connected grid graph. Note that given a disconnected grid graph, one can decompose each connected components separately. A {\em Rectangle-Column-wise aLigned cover (RCL-cover)} (see Figure \ref{fi:niceRCLCOver}) is a partition of $H$ into columns-wise aligned rectangles. The partition is given by a sequence of quadruplets $(c_1^i,c_2^i,r_1^i,r_2^i)_{1\leq i\leq k}$ such that every quadruplet represents a rectangle: A quadruplet $(c_1^i,c_2^i,r_1^i,r_2^i)$ represents the rectangle with $c_{min}=c_1^i,c_{max}=c_2^i,r_{min}=r_1^i,r_{max}=r_2^i$ (that is unique by Observation \ref{obs:Rectangle grid graph is a matrix}). We state the conditions that this sequence of rectangles should follow to be an RCL-cover of $H$ in the following definition.           

\begin{definition}[{\bf Rectangle-Columns-Lined-Up Cover}]\label{def:RCL} 
Let $G=(V,E)$ be a connected grid graph and $H=(V',E')$ be the super rectangle grid graph of $G$. A sequence of quadruplets $(c_1^i,c_2^i,r_1^i,r_2^i)_{1\leq i\leq k}$ is a {\em Rectangle-Column-wise aLigned cover (RCL-cover)} of $H$ if the following conditions are satisfied.
\begin{enumerate}
\item For every $1\leq i\leq k$: $c_2^i>c_1^i$ and $r_2^i>r_1^i$. \label{def:RCL Con1}
\item For every $1\leq i<j\leq k$: if $c_1^i=c_1^j$, then $c_2^i=c_2^j$ and $r_1^j\geq r_2^i$; otherwise, $c_1^j\geq c_2^i$. \label{def:RCL Con2}
\item There exist $1\leq i_1<i_2<\ldots <i_\ell \leq k$ such that $c_1^{i_1}=0$, $c_2^{i_\ell}=c_{max}+1$, and for every $1\leq j<\ell$, it follows that $c_1^{i_{j+1}}=c_2^{i_j}$. \label{def:RCL Con3}
\item For every $1\leq i\leq k$, there exist $\ell \leq i\leq j$ such that $c_1^\ell=c_1^j=c_1^i$, $r_1^\ell=0, r_2^j=r_{max}+1$ and for every $\ell \leq m< j$ it follows that $r_1^{m+1}=r_2^m$. \label{def:RCL Con4}
  

\end{enumerate}    
\end{definition}  

As an example for Definition \ref{def:RCL}, consider the decomposition that is illustrated by Figure \ref{fi:niceRCLCOver}. The sequence of quadruplets $(c_1^i,c_2^i,r_1^i,r_2^i)_{1\leq i\leq 7}$ is given by the rectangles from left-to-right, top-to-bottom. For example, for $i=1$, $c_1^1=0$, $c_2^1=6$, $r_1^1=0$, $r_2^1=5$, and for $i=4$, $c_1^4=13$, $c_2^4=19$, $r_1^4=0$, $r_2^4=6$. We show that the conditions of Definition \ref{def:RCL} are satisfied. Observe that for every rectangle $1\leq i\leq 7$, it follows that $c^i_2>c^i_1$ and $r^i_2>r^i_1$, therefore Condition \ref{def:RCL Con1} is satisfied. Notice that for every two rectangles, $(c_1^i,c_2^i,r_1^i,r_2^i)$ and $(c_1^j,c_2^j,r_1^j,r_2^j)$ for $1\leq i<j\leq 7$, if $c_1^i=c_1^j$, then $(c_1^j,c_2^j,r_1^j,r_2^j)$ is ``located under" $(c_1^i,c_2^i,r_1^i,r_2^i)$, where both of the rectangles have the same right and left ``sides", that is $c_2^i=c_2^j$ and $r_1^j\geq r_2^i$. Otherwise, $(c_1^j,c_2^j,r_1^j,r_2^j)$ is ``located to the right" of $(c_1^i,c_2^i,r_1^i,r_2^i)$, that is, the left ``side" of $(c_1^j,c_2^j,r_1^j,r_2^j)$ is at a column equal or greater then the column that the right ``side" of $(c_1^i,c_2^i,r_1^i,r_2^i)$ is located, so $c_1^j\geq c_2^i$. Therefore, Condition \ref{def:RCL Con2} is satisfied. Now, consider the rectangles that are located at the top, that is, rectangles with $r_1^i=0$; in the example, these are the first, third, fourth and the seventh rectangles in the sequence. Observe that $c_1^1=1, c_2^1=c_1^3, c_2^3=c_1^4, c_2^4=c_1^7, c_2^7=c_{max}+1$, so Condition \ref{def:RCL Con3} is satisfied. Now, given $1\leq i\leq 7$, consider the sub-sequence of rectangles that share the same left and right ``sides". For example, for $i=5$, we have that the $4$-th, $5$-th and the $6$-th rectangles share the same left and right ``sides". Observe that $c_1^4=c_1^5=c^6$, $c_2^4=c_2^5=c_2^6$ and $r_1^4=0, r_2^4=r_1^5, r_2^5-r_1^6, r_2^6=r_{max}+1$, so Condition \ref{def:RCL Con4} is satisfied. Therefore, $(c_1^i,c_2^i,r_1^i,r_2^i)_{1\leq i\leq 7}$ is an RCL-cover of $H$.                     


\begin{figure}[t!]
\centering
\includegraphics[width=0.75\textwidth, page=1]{figures/fig.pdf}
\caption{Example of a nice RCL-cover.}\label{fi:niceRCLCOver}
\end{figure}

Obviously, an RCL-cover of $H$ without additional constrains is not interesting (e.g., one can just cover the entire graph by one rectangle).
Towards imposing additional constrains, given a quadruplet $(c_1^i,c_2^i,r_1^i,r_2^i)$, we now define which vertices of $G$ we include inside the rectangle that $(c_1^i,c_2^i,r_1^i,r_2^i)$ represents. Naturally, every vertex that is (strictly) inside the rectangle ``should" be included. However, notice that two rectangles might share the same ``side"; so, for a vertex that is located on a ``side", we need to decide to which rectangle it belongs. For this purpose, we present the following definition. Intuitively, the term ``$\mathsf{Area}$" denotes the set of vertices of $G$ that are located in a certain ``area" in $H$ (see Figure \ref{fi:area}). For example, $\mathsf{Area}^j$ denotes the set of vertices of $G$ that are located in the $j$-th ``column", and $\mathsf{Area}^{i,j}$ denotes the set of vertices of $G$ that are located between the $i$-th and the $j$-th ``columns", without including the $i$-th ``column". 
More generally, $\mathsf{Area}^{i,j}_{k,\ell}$ denotes the set of vertices of $G$ that are located both $(i)$ between the $i$-th and $j$-th ``columns", without including the $i$-th ``column", and $(ii)$ between the $k$-th and the $\ell$-th ``rows", without including the $k$-th ``row". Formally, we define these as follows.


\begin{definition}\label{def:Vertices in a row}
Given a grid graph $G=(V,E)$ and a super rectangle grid graph $H=(V',E')$ of $G$ with $m$ rows, we define:
\begin{itemize}
\item $\mathsf{Area}^j=\{u_{i,j}\in V$ $:$ $0\leq i\leq m-1$\}.
\item $\mathsf{Area}_k^{i,j}=\{u_{k,t}\in V$ $:$ $i<t\leq j$\}.
\item $\mathsf{Area}^{i,j}=\bigcup^{j}_{t=i+1}\mathsf{Area}^t$.

\item $\mathsf{Area}^i_{k,\ell}=\{u_{t,i}\in V$ $:$ $k<t \leq \ell$\}.
\item $\mathsf{Area}^{i,j}_{k,\ell}=\bigcup^{j}_{t=i+1}\mathsf{Area}^t_{k,\ell}$.
\end{itemize}

\end{definition}

\begin{figure}[t!]
\centering
\includegraphics[width=0.75\textwidth, page=4]{figures/fig.pdf}
\caption{Example for some of the notations of Definition \ref{def:Vertices in a row}. The vertices of the set $\mathsf{Area}^{c_0}$ are marked in orange. The vertices of $\mathsf{Area}^{c_1,c_2}_{r_1}$ are marked in purple, where the columns $\mathsf{Area}^{c_1}$ and $\mathsf{Area}^{c_2}$ of $H$ are highlighted in yellow. The vertices of $\mathsf{Area}^{c_2,c_3}_{r_1,r_2}$ are marked in pink and orange, where the columns $\mathsf{Area}^{c_2}$ and $\mathsf{Area}^{c_3}$ and the rows $\mathsf{Area}^{c_2,c_3}_{r_1}$ and $\mathsf{Area}^{c_2,c_3}_{r_2}$ of $H$, are highlighted in yellow and orange.}\label{fi:area}
\end{figure}

As $\mathsf{Area}^j$ is the set of all the vertices located at the $j$-th column, we call $\mathsf{Area}^j$ a {\em column}. On the other hand, $\mathsf{Area}_i^{k,\ell}$ contains vertices from the $i$-th row but not necessary all of them. For our purposes, we still call $\mathsf{Area}_i^{k,\ell}$ a {\em row}, for every $k$ and $\ell$.  % Observe that every vertex $v\in V$ that is not on the boundary of one of the rectangles, belongs to exactly one rectangle. 
% Observe that an RCL-cover $(c_1^i,c_2^i,r_1^i,r_2^i)_{1\leq i\leq k}$ generates a naturally partition of the graph $G$ to $k$ disjoint sets. Every vertex $u\in V$ belongs to exactly one rectangle.

 Next, we define the constraints that our decomposition should satisfy. For now, we define them for a general sequence of subsets $(U_i)_{1\leq i\leq k}$ of $V$, and later we define them for an RCL-cover. Inuitively, a {\em nice decomposition} of $G$ is a partition of $V$ into a sequence of disjoint subsets $(U_i)_{1\leq i\leq k}$ of $V$ such that every $U_i$ contains $\Theta(\sqrt{n})$ vertices, and for every $1\leq i \leq k$, the size of the boundary of $\bigcup_{1\leq \ell \leq i}U_\ell$ is bounded by $\OO(\sqrt{n})$.    


\begin{definition}[{\bf Nice Decomposition}]\label{def:niceDe} 
A {\em nice decomposition} of a connected grid graph $G=(V,E)$ is a sequence of subsets of $V$, $(U_i)_{1\leq i\leq k}$, that satisfies the following conditions.
\begin{enumerate}
\item For every $v\in V(G)$: there exists $1\leq i\leq k$ such that $v\in U_i$. \label{dcon1}
\item For every $1\leq i,j \leq k, i\neq j$: $U_i \cap U_j=\emptyset$. \label{dcon2}
\item For every $1\leq i \leq k$: $\sqrt{n}\leq |U_i|\leq 6\sqrt{n}$. \label{dcon3}
\item For every $1\leq i \leq k$: $|B(\bigcup_{1\leq \ell \leq i}U_\ell)|\leq 5\sqrt{n}$. \label{dcon4}
\end{enumerate}

\end{definition}      

%\begin{itemize}
%\item 
%\item 
%\end{itemize}



We are now ready to define formally what decomposition we aim to construct called a {\em nice RCL-cover} (see Figure \ref{fi:niceRCLCOver}). From a geometric perspective, we would like to partition of $H$ (the super rectangle grid graph of $G$), into column-wise aligned rectangles, that is, an RCL-cover of $H$ (see Definition \ref{def:RCL}). In addition, we would like the subsets of vertices ``corresponding'' to the RCL-cover to satisfy the conditions in Definition \ref{def:niceDe}.    


\begin{definition}[{\bf Nice RCL-cover}]\label{def:niceRCLDe} 
Let $G=(V,E)$ be a connected grid graph and let $H$ be a super rectangle grid graph of $G$. An RCL-cover of $H$, $(c_1^i,c_2^i,r_1^i,r_2^i)$ $_{1\leq i\leq k}$, is a nice decomposition of $G$ if $(\mathsf{Area}^{c_1^i,c_2^i}_{r_1^i,r_2^i})_{1\leq i\leq k}$ is a nice decomposition of $G$.
\end{definition}
  
\section{Computation of (Almost) Nice Columns and Rows} \label{section nice C and R}
Having defined our objective explicitly (computing a nice RCL-cover in linear time), we would like to pursue it. We begin with a simple observation regarding the graph $H$, which will be useful later.    


\begin{observation} \label{obs:Good super rectangle grid graph}
Given a connected grid graph $G=(V,E)$ with $n$ vertices and its super rectangle grid graph $H$, the following conditions are satisfied: 
\begin{enumerate}
\item\label{condition:1n+2row&column} $H$ has $r_{max}+2$ rows and $c_{max}+2$ columns.
\item\label{condition:2first&lastRempty} $\mathsf{Area}^0=\mathsf{Area}^{c_{max}+1}=\mathsf{Area}^{0,c_{max}+1}_0=\mathsf{Area}^{0,c_{max}+1}_{r_{max}+1}=\emptyset$.
\item\label{condition:3C1nonempty}  $\mathsf{Area}^1\neq \emptyset$.
\end{enumerate}
\end{observation}

Towards our construction of a nice RCL-cover, we would first like to find a certain partition of $H$ into ``large" rectangles, separated by columns. More precisely, we would like to find a certain sequence of $t$ columns, $(\mathsf{Area}^{i_j})_{1\leq j\leq t}$, such that $0=i_1<i_2<\ldots<i_t=c_{max}+1$. Here, every pair $(\mathsf{Area}^{i_j},\mathsf{Area}^{i_{j+1}})$ represents the rectangle with $r'_{min}=0,r'_{max}=r_{max}+1,c'_{min}=i_j,c'_{max}=i_{j+1}$. We will find this partition using induction, beginning with the first column, $\mathsf{Area}^0$. Now, assume that the previous column we found is $\mathsf{Area}^i$. In the next definition, we state the conditions that the next column should satisfy with respect to the previous one: the next column, $\mathsf{Area}^j$, should contain $\OO(\sqrt{n})$ vertices from $G$, the number of vertices between $\mathsf{Area}^j$ and the previous column $\mathsf{Area}^i$ should be $\Omega(\sqrt{n})$, and $\mathsf{Area}^j$ should be relatively ``close" to $\mathsf{Area}^i$. Then, we say that $\mathsf{Area}^j$ is {\em nice} with respect to $\mathsf{Area}^i$ (see Figure \ref{fi:niceColumns}):

\begin{definition} [{\bf Nice Column}] \label{def:Nice column}
Given a connected grid graph $G=(V,E)$ with $n$ vertices and $H=(V',E')$, the columns of $H$ are classified as {\em nice} or {\em not nice} as follows. First, $\mathsf{Area}^0$ is nice. For $0\leq i<j\leq c_{max}+1$, $\mathsf{Area}^j$ is nice with respect to $\mathsf{Area}^i$ if the following conditions are satisfied.
\begin{enumerate}
\item\label{condition:1numincolumn} $|\mathsf{Area}^j|\leq \sqrt{n}$.
\item\label{condition:2numinsumcolumn} $|\mathsf{Area}^{i,j}|\geq \sqrt{n}$.
\item\label{condition:3distancefrom last} $j-i\leq 2\sqrt{n}$.
\end{enumerate}
\end{definition}


\begin{figure}[t!]
\centering
\includegraphics[width=0.75\textwidth, page=2]{figures/fig.pdf}
\caption{Example of nice columns. In this graph, $n=81$ and $\sqrt{n}=9$. For $1\leq i\leq 3$, $\mathsf{Area}^{nc_{i+1}}$ is a nice column with respect to $\mathsf{Area}^{nc_{i}}$. Moreover, $\mathsf{Area}^{nc'_{5}}$ is a nice column with respect to $\mathsf{Area}^{nc_{4}}$ and $\mathsf{Area}^{nc_{5}}$ is an almost nice column with respect to $\mathsf{Area}^{nc_{4}}$. For example, $|\mathsf{Area}^{nc_1,nc_2}|=21$, so $|\mathsf{Area}^{nc_1,nc_2}|\geq \sqrt{n}$, therefore Condition \ref{condition:1numincolumn} is satisfied. Because $\mathsf{Area}^{nc_2}=3\leq 9=\sqrt{n}$, Condition \ref{condition:2numinsumcolumn} is satisfied. Because $nc_2-nc_1=6\leq 18=2\sqrt{n}$, Condition \ref{condition:3distancefrom last} is satisfied. Therefore, $\mathsf{Area}^{nc_{2}}$ is a nice column with respect to $\mathsf{Area}^{nc_{1}}$.}\label{fi:niceColumns}
\end{figure}

In the following lemma we prove the existence of a nice column $\mathsf{Area}^j$ with respect to $\mathsf{Area}^i$ if there are ``enough" vertices to its ``right", that is, if $|\mathsf{Area}^{i,c_{max}+1}|\geq \sqrt{n}$.


\begin{lemma}\label{lem:Nice column}
Let $G=(V,E)$ be a connected grid graph  with $n$ vertices, let $H=(V',E')$ be its super rectangle grid graph, and let $\mathsf{Area}^i$ be a column. If $i<c_{max}+1$ and $|\mathsf{Area}^{i,c_{max}+1}|\geq \sqrt{n}$, then there exists $i<j\leq c_{max}+1$ such that $\mathsf{Area}^j$ is nice with respect to $\mathsf{Area}^i$.
\end{lemma}  

\begin{proof}
First, we show that $\mathsf{Area}^{i+1}\neq \emptyset$. If $i=0$, then this is true because by Condition \ref{condition:3C1nonempty} of Observation \ref{obs:Good super rectangle grid graph}, we know that $\mathsf{Area}^1\neq \emptyset$. Otherwise, $i\geq 1$. Since $\mathsf{Area}^1\neq \emptyset$, $|\mathsf{Area}^{i,c_{max}+1}|\geq \sqrt{n}\geq 1$ and $G$ is connected, we get that $\mathsf{Area}^{i+1}\neq \emptyset$. Now, there must be $i<k<i+\sqrt{n}+1$ such that $|\mathsf{Area}^{i,k}|\geq \sqrt{n}$; otherwise, there exists $i<m<i+\sqrt{n}+1$ such that $\mathsf{Area}^m=\emptyset$ and $\mathsf{Area}^{m,c_{max}+1}\neq \emptyset$, which contradicts $G$'s connectivity. Now, we claim that there must be $k\leq \ell \leq k+\sqrt{n}$ such that $|\mathsf{Area}^{\ell} |\leq \sqrt{n}$. Towards a contradiction, assume that there is no such $\ell$. Therefore, for each $k\leq \ell \leq k+\sqrt{n}$, we get that $|\mathsf{Area}^{\ell} |\geq \sqrt{n}+1$, so $|\mathsf{Area}^{k,k+\sqrt{n}}|> \sqrt{n}\cdot \sqrt{n}=n$, a contradiction. We claim that $\mathsf{Area}^{\ell}$ is a nice column with respect to $\mathsf{Area}^i$. Condition \ref{condition:1numincolumn} is satisfied by the definition of $\mathsf{Area}^{\ell}$. Condition \ref{condition:2numinsumcolumn} is satisfied because $k\leq \ell$ implies $\mathsf{Area}^{i,k}\subseteq \mathsf{Area}^{i,\ell}$. Therefore, $|\mathsf{Area}^{i,k}|\geq \sqrt{n}$ implies $|\mathsf{Area}^{i,\ell} |\geq \sqrt{n}$. Moreover, $\ell -i\leq k+\sqrt{n}-i\leq \sqrt{n}+i+\sqrt{n}-i=2\sqrt{n}$, so Condition \ref{condition:3distancefrom last} is satisfied. Thus, $\mathsf{Area}^{\ell}$ is a nice column with respect to $\mathsf{Area}^i$.             
\end{proof}

We continue with the discussion of finding a partition of $H$ into ``large" rectangles, separated by columns, by induction. In Lemma \ref{lem:Nice column} we proved the existence of a nice column $\mathsf{Area}^j$ with respect to $\mathsf{Area}^i$ if $|\mathsf{Area}^{i,c_{max}+1}|\geq \sqrt{n}$. We now want to handle the case where we consider a nice column $\mathsf{Area}^j$ and $|\mathsf{Area}^{j,c_{max}+1}|< \sqrt{n}$. In this case instead of $\mathsf{Area}^j$, we take the last column in $H$, $\mathsf{Area}^{c_{max}+1}$, as the last column in our partition. Observe that in this case, Condition \ref{condition:3distancefrom last} in Definition \ref{def:Nice column} might not be satisfied, so $\mathsf{Area}^{c_{max}+1}$ might not be a nice column with respect to $\mathsf{Area}^{i}$; but, as we will see later, it will still good enough for our purposes. Specifically, in this case, we say that $\mathsf{Area}^{c_{max}+1}$ is an {\em almost nice column} with respect to $\mathsf{Area}^{i}$ (see Figure \ref{fi:niceColumns}). We generalize this definition to capture more than only the last column $\mathsf{Area}^{c_{max}+1}$ (the reason for that will be clear later).        

\begin{definition} [{\bf Almost Nice Column}]\label{def:almost nice column}
For a connected grid graph $G=(V,E)$ with $n$ vertices and $H=(V',E')$, columns are classified as {\em almost nice} or not as follows. First, we say that $\mathsf{Area}^0$ is almost nice. For $0<i<j\leq c_{max}+1$ we say that $\mathsf{Area}^j$ is almost nice with respect to $\mathsf{Area}^i$ if the following conditions are satisfied:
\begin{enumerate}
\item\label{condition:1numinNcolumn} $|\mathsf{Area}^j|\leq \sqrt{n}$.
\item\label{condition:2numinNsumcolumn} $|\mathsf{Area}^{i,j}|\geq \sqrt{n}$.
\item\label{condition:3niceisinside} There exists $i<k\leq j$ such that $\mathsf{Area}^k$ is nice with respect to $\mathsf{Area}^i$ and $|\mathsf{Area}^{k,j}|<\sqrt{n}$.
\end{enumerate}
\end{definition}

Later, after we have the partition of $H$ into ``large" rectangles, we will get a partition of every ``large" rectangle into ``smaller" rectangles. For that purpose, we want every row of every rectangle to contain $\OO(\sqrt{n})$ vertices. Observe that we derive this constraint from Condition \ref{condition:3niceisinside} of Definition \ref{def:almost nice column}.      

Observe that if $\mathsf{Area}^j$ is a nice column with respect to $\mathsf{Area}^i$, then $\mathsf{Area}^j$ is also an almost nice column with respect to $\mathsf{Area}^i$. Moreover, if $\mathsf{Area}^j$ is a nice column with respect to $\mathsf{Area}^i$ and $\mathsf{Area}^{j,c_{max}+1}<\sqrt{n}$ then $\mathsf{Area}^{c_{max}+1}$ is an almost nice column with respect to $\mathsf{Area}^i$. We state these insights in the next two observations. 

\begin{observation}\label{obs:nice is almost}
Every nice column $\mathsf{Area}^j$ with respect to $\mathsf{Area}^i$ is also an almost nice column with respect to $\mathsf{Area}^i$.
\end{observation} 

\begin{observation}\label{obs:n+1 is almost}
Assume that $\mathsf{Area}^j$ is a nice column with respect to $\mathsf{Area}^i$ and $\mathsf{Area}^{j,c_{max}+1}<\sqrt{n}$. Then, $\mathsf{Area}^{c_{max}+1}$ is an almost nice column with respect to $\mathsf{Area}^i$.
\end{observation}

Now, assume that we have a partition of $H$ into ``large" rectangles separated by columns, and let $\mathsf{Area}^i$ and $\mathsf{Area}^j$ be two columns in the partition such that $\mathsf{Area}^j$ is also an almost nice column with respect to $\mathsf{Area}^i$. We would like to have a partition of the ``large" rectangle, defined by $r'_{min}=0,r'_{max}=r_{max}+1,c_{min}=i,c_{max}=j$ into ``smaller" rectangles having $\mathsf{Area}^i$ and $\mathsf{Area}^j$ as their left and right ``sides". Thus, we need to partition of the ``area" between $\mathsf{Area}^i$ and $\mathsf{Area}^j$ by using rows as ``sides". With a search similar to the search for a nice column, we will find such a partition by induction. The first row is $\mathsf{Area}^{i,j}_{0}$. Now, assume that the previous row we found is $\mathsf{Area}^{i,j}_{k}$, and we seek the next row. In the following definition, we state the conditions we want the next row to satisfy with respect to the previous one. Briefly, we want the next row, $\mathsf{Area}^{i,j}_{\ell}$, to contain $\OO(\sqrt{n})$ vertices from $G$, and the number of vertices between $\mathsf{Area}^{i,j}_{\ell}$ and the previous row $\mathsf{Area}^{i,j}_{k}$ to be at least $\sqrt{n}$ but not more than $5\sqrt{n}$. If $\mathsf{Area}^{i,j}_{\ell}$ is such a row, we say that $\mathsf{Area}^{i,j}_{\ell}$ is {\em nice} with respect to $\mathsf{Area}^{i,j}_{k}$ (see Figure \ref{fi:niceRow}).
           
%    such that we satisfy the conditions of a nice RCL-cover, if we do that for every two successive columns we found. Th Similar to the search for the nice column, we find the $\mathsf{Area}^{i,j}$ into rows, so together with $\mathsf{Area}^i$ and $\mathsf{Area}^j$ we get a partition of the ``area" between these two columns, to rectangles.  we can get our nice RCL-cover

\begin{definition}[{\bf Nice Row}] \label{def:Nice Row}
For a connected grid graph $G=(V,E)$ with $n$ vertices, its super rectangle grid graph $H$, and two columns $\mathsf{Area}^i$ and $\mathsf{Area}^j$ for $i<j$, the rows of $H$ are classified as {\em nice} or not nice as follows. First, $\mathsf{Area}_{0}^{i,j}$ is nice. For $0\leq k<\ell \leq r_{max}+1$, $\mathsf{Area}_{\ell}^{i,j}$ is nice with respect to $\mathsf{Area}_k^{i,j}$ if and only if the following conditions are satisfied:
\begin{enumerate}
\item\label{condition:1numinrow} $|\mathsf{Area}_{\ell}^{i,j}|\leq 3\sqrt{n}$.
\item\label{condition:2numinsumrows} $\sqrt{n}\leq |\mathsf{Area}_{k,\ell}^{i,j}|\leq 5\sqrt{n}$.
\end{enumerate}
\end{definition}


\begin{figure}[t!]
\centering
\includegraphics[width=0.75\textwidth, page=3]{figures/fig.pdf}
\caption{Example of nice rows. In this graph, $n=81$ and $\sqrt{n}=9$. The nice columns are highlighted in yellow. The nice rows are highlighted in blue. For example, $|\mathsf{Area}_{nr_2}^{nc_1,nc_2}|=5\leq 27=3\sqrt{n}$, so Condition \ref{condition:1numinrow} is satisfied. Because $|\mathsf{Area}_{nr_1,nr_2}^{nc_1,nc_2}|=11$, $\sqrt{n}\leq|\mathsf{Area}_{nr_1,nr_2}^{nc_1,nc_2}|\leq 5\sqrt{n}$, so Condition \ref{condition:2numinsumrows} is satisfied. Therefore, $\mathsf{Area}_{nr_2}^{nc_1,nc_2}$ is a nice row with respect to $\mathsf{Area}_{nr_1}^{nc_1,nc_2}$.}\label{fi:niceRow}
\end{figure}


In the next lemma, we prove the existence of a nice row $\mathsf{Area}_{p}^{i,j}$ with respect to $\mathsf{Area}_{k}^{i,j}$, given that $\mathsf{Area}^j$ is an almost nice column with respect to $\mathsf{Area}^i$ and if we have ``enough" vertices ``below", that is, if $|\mathsf{Area}_{k,r_{max}+1}^{i,j}|\geq \sqrt{n}$.

\begin{lemma}\label{lem:nice row} Let $G=(V,E)$ be a connected grid graph with $n$ vertices, let $H$ be its super rectangle grid graph, let $\mathsf{Area}^j$ be an almost nice column with respect to $\mathsf{Area}^i$, and let $\mathsf{Area}_{k}^{i,j}$ be a row. If $|\mathsf{Area}_{k,r_{max}+1}^{i,j}|\geq \sqrt{n}$, then there exists $k<p\leq r_{max}+1$ such that $\mathsf{Area}_{p}^{i,j}$ is nice with respect to $\mathsf{Area}_{k}^{i,j}$. 
\end{lemma}

\begin{proof}
Towards a contradiction, assume that there does not exist such a $p$. As $|\mathsf{Area}_{k,r_{max}+1}^{i,j}|\geq \sqrt{n}$, there exists $k<p'<r_{max}+1$ such that $|\mathsf{Area}_{k,p'}^{i,j}|\geq \sqrt{n}$. Let $p$ be the smallest such index $p'$. As $\mathsf{Area}_{p}^{i,j}$ is not nice with respect to $\mathsf{Area}_{k}^{i,j}$, at least one of the two conditions of Definition \ref{def:Nice Row} is false. First, assume that Condition \ref{condition:1numinrow} is not true. As $\mathsf{Area}^j$ is almost nice with respect to $\mathsf{Area}^i$, there exists $i<t\leq j$ such that $\mathsf{Area}^t$ is nice with respect to $\mathsf{Area}^i$ and $|\mathsf{Area}^{t,j}|<\sqrt{n}$. Notice that for every $0\leq a\leq r_{max}+1$, we get that $\mathsf{Area}_{a}^{t,j}\subseteq \mathsf{Area}_{0,r_{max}+1}^{t,j}=\mathsf{Area}^{t,j}$, which implies $|\mathsf{Area}_{a}^{t,j}|\leq |\mathsf{Area}^{t,j}|<\sqrt{n}$. By Condition \ref{condition:3niceisinside} of Definition \ref{def:Nice column}, we know that $t-i\leq 2\sqrt{n}$, which implies that $|\mathsf{Area}_{p}^{i,t}|\leq 2\sqrt{n}$. Notice that $\mathsf{Area}_{p}^{i,j}=\mathsf{Area}_{p}^{i,t}\cup \mathsf{Area}_{p}^{t,j}$, which implies $|\mathsf{Area}_{p}^{i,j}|\leq |\mathsf{Area}_{p}^{i,t}|+ |\mathsf{Area}_{p}^{t,j}|$. Therefore, $|\mathsf{Area}_{p}^{i,j}|\leq 2\sqrt{n}+ \sqrt{n}=3\sqrt{n}$, a contradiction. Now, assume that Condition \ref{condition:2numinsumrows} is false. Note that $|\mathsf{Area}_{k,p}^{i,j}|\geq \sqrt{n}$. Therefore, the assumption that Condition \ref{condition:2numinsumrows} is not true means that $5\sqrt{n}<|\mathsf{Area}_{k,p}^{i,j}|$. Notice that $\mathsf{Area}_{k,p-1}^{i,j}=\mathsf{Area}_{k,p}^{i,j}\setminus \mathsf{Area}_{p}^{i,j}$, which implies $|\mathsf{Area}_{k,p-1}^{i,j}|\geq |\mathsf{Area}_{k,p}^{i,j}|-|\mathsf{Area}_{p}^{i,j}|$. We saw that $|\mathsf{Area}_{p}^{i,j}|\leq 3\sqrt{n}$, so we get $|\mathsf{Area}_{k,p-1}^{i,j}|\geq |\mathsf{Area}_{k,p}^{i,j}|-|\mathsf{Area}_{p}^{i,j}|\geq 5\sqrt{n}-3\sqrt{n}=2\sqrt{n}$, a contradiction to the minimality of $p$. Either way, we got a contradiction, so the lemma stands.        
\end{proof} 

In Lemma \ref{lem:nice row}, we proved the existence of a nice row $\mathsf{Area}_{p}^{i,j}$ with respect to $\mathsf{Area}_{k}^{i,j}$ if $|\mathsf{Area}_{k,r_{max}+1}^{i,j}|\geq \sqrt{n}$. Now, we want to handle the case where we find the next nice row $\mathsf{Area}_{p}^{i,j}$ and $|\mathsf{Area}_{p,r_{max}+1}^{i,j}|< \sqrt{n}$. In this case, instead of $\mathsf{Area}_{p}^{i,j}$, we take the last row in $\mathsf{Area}^{i,j}$ as the last row that defines our partition to rectangles of $\mathsf{Area}^{i,j}$, that is, $\mathsf{Area}^{i,j}_{r_{max}+1}$. Observe that in this case, Condition \ref{condition:2numinsumrows} might not be satisfied, so $\mathsf{Area}^{i,j}_{r_{max}+1}$ might not be a nice row with respect to $\mathsf{Area}_{k}^{i,j}$; however, it will still be good enough for our purposes. In this case, we say that $\mathsf{Area}_{p}^{i,j}$ is an {\em almost nice row} with respect to $\mathsf{Area}_{k}^{i,j}$. We generalize this definition beyond the last row $\mathsf{Area}^{i,j}_{r_{max}+1}$ (the reason for that will be clear later):

\begin{definition}[{\bf Almost Nice Row}] \label{def:Almost Nice Row}
For a connected grid graph $G=(V,E)$ with $n$ vertices, its super rectangle grid graph $H$, and two columns $\mathsf{Area}^i$ and $\mathsf{Area}^j$ with $i<j$, the rows of $H$ are classified as {\em almost nice} or {\em not almost nice} as follows. First, $\mathsf{Area}_{0}^{i,j}$ is almost nice. For $0\leq k<\ell \leq r_{max}+1$, $\mathsf{Area}_{\ell}^{i,j}$ is almost nice with respect to $\mathsf{Area}_k^{i,j}$ if and only if the following conditions are satisfied:
\begin{enumerate}
\item\label{condition:1numinArow} $|\mathsf{Area}_{\ell}^{i,j}|\leq 3\sqrt{n}$.
\item\label{condition:2numinsumArows} $\sqrt{n}\leq |\mathsf{Area}_{k,\ell}^{i,j}|\leq 6\sqrt{n}$.
\end{enumerate}
\end{definition}      

Observe that if $\mathsf{Area}_{p}^{i,j}$ is a nice row with respect to $\mathsf{Area}_{k}^{i,j}$, $\mathsf{Area}_{p}^{i,j}$ is also an almost nice row with respect to $\mathsf{Area}_{k}^{i,j}$. Moreover, if $\mathsf{Area}_{p}^{i,j}$ is a nice row with respect to $\mathsf{Area}_{k}^{i,j}$ and $|\mathsf{Area}_{p,r_{max}+1}^{i,j}|< \sqrt{n}$, then $\mathsf{Area}_{r_{max}+1}^{i,j}$ is an almost nice row with respect to $\mathsf{Area}_{k}^{i,j}$. We state these insights in the observations ahead. 

\begin{observation}\label{obs:nice row is almost}
Every nice row $\mathsf{Area}_{p}^{i,j}$ with respect to $\mathsf{Area}_{k}^{i,j}$ is also an almost nice row with respect to $\mathsf{Area}_{k}^{i,j}$.
\end{observation} 

\begin{observation}\label{obs:n+1 is almost row}
Assume that $\mathsf{Area}_{p}^{i,j}$ is a nice row with respect to $\mathsf{Area}_{k}^{i,j}$ and $|\mathsf{Area}_{p,r_{max}+1}^{i,j}|< \sqrt{n}$. Then, $\mathsf{Area}_{r_{max}+1}^{i,j}$ is an almost nice row with respect to $\mathsf{Area}_{k}^{i,j}$.
\end{observation}

Later, we will prove the existence of some conditions regarding to nice columns and rows and almost nice columns and rows. Due to Observations \ref{obs:nice is almost} and \ref{obs:nice row is almost}, it is enough to prove these conditions for almost nice columns and rows.

Now, we use our definitions of a nice column and a nice row to construct a nice RCL-cover of $G$. In particular, we show that if $(c_1^i,c_2^i,r_1^i,r_2^i)_{1\leq i\leq k}$ is an RCL-cover of $H$ such that for every $1\leq i\leq k$, $\mathsf{Area}^{c_2^i}$ is an almost nice column with respect to $\mathsf{Area}^{c_1^i}$ and $\mathsf{Area}^{c_1^i,c_2^i}_{r_2^i}$ is an almost nice row with respect to $\mathsf{Area}^{c_1^i,c_2^i}_{r_1^i}$, then $(c_1^i,c_2^i,r_1^i,r_2^i)_{1\leq i\leq k}$ is also a nice RCL-cover of $G$. We prove this statement in Lemma \ref{lem:niceRCL} ahead. Towards that, we begin with a simple observation that will be used in the proof.     


\begin{observation} \label{obs:emptyS}
Let $G=(V,E)$ be a connected grid graph, and let $H=(V',E')$ be its super rectangle grid graph. Let $(c_1^i,c_2^i,r_1^i,r_2^i)_{1\leq i\leq k}$ be an RCL-cover of $H$. Then, for every $1\leq i,j \leq k$ such that $i\neq j$, it follows that $\mathsf{Area}^{c_1^i,c_2^i}_{r_1^i,r_2^i} \cap \mathsf{Area}^{c_1^j,c_2^j}_{r_1^j,r_2^j} =\emptyset$. 
\end{observation}

\begin{lemma}\label{lem:niceRCL}
Let $G=(V,E)$ be a connected grid graph, and let $H=(V',E')$ be its super rectangle grid graph. Let $(c_1^i,c_2^i,r_1^i,r_2^i)_{1\leq i\leq k}$ be an RCL-cover of $H$. Suppose that for every $1\leq i\leq k$, $\mathsf{Area}^{c_2^i}$ is an almost nice column with respect to $\mathsf{Area}^{c_1^i}$, and $\mathsf{Area}^{c_1^i,c_2^i}_{r_2^i}$ is an almost nice row with respect to $\mathsf{Area}^{c_1^i,c_2^i}_{r_1^i}$. Then, $(c_1^i,c_2^i,r_1^i,r_2^i)_{1\leq i\leq k}$ is a nice RCL-cover of $G$. 
\end{lemma}

In order to make the proof of Lemma \ref{lem:niceRCL} below easier to read, we will denote $\mathsf{Area}^{c_1^i,c_2^i}_{r_1^i,r_2^i}$ by $\mathsf{Area}(i)$.

\begin{proof}
We need to show that the conditions of Definition \ref{def:niceDe} are satisfied.
Let $v\in V(G)$. Then, $v=u_{r,c}$ for some $0\leq r \leq r_{max}+1$ and $0\leq c \leq c_{max}+1$. First, notice that for every $1\leq i<j\leq k$, it follows that $c_1^i<c_2^i\leq c_1^j<c_2^j$. As $c_1^1=0$ and $c_2^k=c_{max}+1$, there exists $1\leq i\leq k$ such that $c_1^i\leq c \leq c_2^i$. Now, notice that for every $c_1,c_2$, if there exists $i$ such that $c_1^i=c_1$ and $c_2^i=c_2$, then there exist $s\leq i\leq t$ such that $c_1^s=c_1^t=c_1$, $c_2^s=c_2^t=c_2$, $r_1^s=0$ and $r_2^t=r_{max}+1$. Moreover, for every $s\leq \ell<m \leq t$ it follows that $c_1^\ell=c_1^m=c_1$, $c_2^\ell=c_2^m=c_2$ and $r_1^\ell<r_2^\ell \leq r_1^m<r_2^m$. Therefore, there must be some $s\leq \ell \leq t$ such that $r_1^\ell \leq r\leq r_2^\ell$. Thus we get that $v\in \mathsf{Area}(\ell)$, so Condition \ref{dcon1} of Definition \ref{def:niceDe} is satisfied.


Condition \ref{dcon2} of Definition \ref{def:niceDe} is satisfied due to Observation \ref{obs:emptyS}.

Let $1\leq i\leq k$. We have that $\mathsf{Area}^{c_1^i,c_2^i}_{r_2^i}$ is an almost nice row with respect to $\mathsf{Area}^{c_1^i,c_2^i}_{r_1^i}$. Therefore, by Definition \ref{def:Almost Nice Row}, we get that $\sqrt{n} \leq \mathsf{Area}^{c_1^i,c_2^i}_{r_1^i,r_2^i}\leq 6\sqrt{n}$. So, Condition \ref{dcon3} of Definition \ref{def:niceDe} is satisfied as well.   


Again, let $1\leq i\leq k$. We next show that $\bigcup_{1\leq \ell \leq i}\mathsf{Area}(\ell)=\mathsf{Area}^{0,c_1^i}\cup \mathsf{Area}^{c_1^i,c_2^i}_{0,r_2^i}$. Let $v\in \bigcup_{1\leq \ell \leq i}\mathsf{Area}(\ell)$. Let $1\leq \ell \leq i$ be such that $v\in \mathsf{Area}(\ell)$. If $c_1^\ell\neq c_1^i$, then since $(c_1^i,c_2^i,r_1^i,r_2^i)_{1\leq i\leq k}$ is an RCL-cover of $H$, by Definition \ref{def:RCL} we get that $c_2^\ell \leq c_1^i$, so $v\in \mathsf{Area}^{0,c_1^i}$. Otherwise, $c_1^\ell=c_1^i$, and by Definition \ref{def:RCL}, we get that $c_2^\ell=c_2^i$ and $r_2^\ell \leq r_2^i$, so $v\in \mathsf{Area}^{c_1^i,c_2^i}_{0,r_2^i}$. Now, let $v\in \mathsf{Area}^{c_1^i,c_2^i}_{0,r_2^i}$. So, $v=u_{r,c}$ for some $0\leq r\leq r_2^i$ and $c_1^i<c\leq c_2^i$. From Definition \ref{def:RCL} we get that there exists $1\leq \ell \leq i$ such that $c_1^\ell=c_1^i$,$c_2^\ell=c_2^i$ and $r_1^\ell<r\leq r_2^\ell$, so $v\in \mathsf{Area}(\ell)$. Similarly, let $v\in \mathsf{Area}^{0,c_1^i}$. So, $v=u_{r,c}$ for some $0\leq r\leq r_{max}+1$ and $0<c\leq c_1^i$. By Definition \ref{def:RCL}, there exists $1\leq \ell \leq i$ such that $c_1^\ell<c\leq c_2^\ell$ and $r_1^\ell<r\leq r_2^\ell$, so $v\in \mathsf{Area}(\ell)$. Therefore, we get that $\bigcup_{1\leq \ell \leq i}\mathsf{Area}(\ell))=\mathsf{Area}^{0,c_1^i}\cup \mathsf{Area}^{c_1^i,c_2^i}_{0,r_2^i}$. It is easy to see that $B(\bigcup_{1\leq \ell \leq i}\mathsf{Area}(\ell))=B(\mathsf{Area}^{0,c_1^i}\cup \mathsf{Area}^{c_1^i,c_2^i}_{0,r_2^i})\subseteq \mathsf{Area}^{c_1^i}\cup \mathsf{Area}^{c_2^i}\cup \mathsf{Area}^{c_1^i,c_2^i}_{r_2^i}$. Now, since $\mathsf{Area}^{c_1^i}$ and $\mathsf{Area}^{c_2^i}$ are almost nice columns (with respect to some columns), and $\mathsf{Area}^{c_1^i,c_2^i}_{r_2^i}$ is an almost nice row (with respect to some row) we get that $|\mathsf{Area}^{c_1^i}|+|\mathsf{Area}^{c_2^i}|+|\mathsf{Area}^{c_1^i,c_2^i}_{r_2^i}|\leq 5\sqrt{n}$. Therefore, we get that $|B(\bigcup_{1\leq \ell \leq i}\mathsf{Area}(\ell))|\leq 5\sqrt{n}$, so Condition \ref{dcon4} is satisfied.
%       Now $\mathsf{Area}^{c_1^i,c_2^i}_{r_2^i}$ is a nice row with respect to $\mathsf{Area}^{c_1^i,c_2^i}_{r_1^i}$. Therefore, by definition $\sqrt{n}\leq |\mathsf{Area}(i)|\leq 5\sqrt{n}$, so Condition \ref{dcon3} is satisfied. 

%Let $1\leq i \leq k-1$. Now, if $r_1^{i+1}=0$ then $B(\bigcup_{1\leq \ell \leq i}\mathsf{Area}(\ell))\cap \mathsf{Area}(i+1)\subseteq \mathsf{Area}^{c_2^i}\cap \mathsf{Area}(i+1)\subseteq B(\bigcup_{1\leq \ell \leq i} \mathsf{Area}(i+1))\cap B(\mathsf{Area}(i+1))$.

%If $r_1^{i+1}\neq 0$, then $(\bigcup_{1\leq \ell \leq i}\mathsf{Area}(\ell))\cap \mathsf{Area}(i+1)\subseteq (\mathsf{Area}^{c_2^i}\cap \mathsf{Area}(i+1))\cup \mathsf{Area}^{c_1^{i+1},c_2^{i+1}}_{r_1^{i+1}} \subseteq B(\bigcup_{1\leq \ell \leq i} \mathsf{Area}(\ell))\cap B(\mathsf{Area}(i+1))$.
%Therefore the third condition holds.

%Let $1\leq i \leq k-1$. Notice that $B((\bigcup_{1\leq \ell \leq i} \mathsf{Area}(\ell)) \cup \mathsf{Area}(i+1))\subseteq  \mathsf{Area}^{c_1^{i+1}}\cup \mathsf{Area}^{c_2^{i+1}}\cup \mathsf{Area}^{c_1^{i+1},c_2^{i+1}}_{r_2^{i+1}}$. Since $\mathsf{Area}^{c_1^{i+1}}, \mathsf{Area}^{c_2^{i+1}}$ are almost nice columns (with respect to some columns), and $\mathsf{Area}^{c_1^{i+1},c_2^{i+1}}_{r_2^{i+1}}$ is a nice row (with respect to $\mathsf{Area}^{c_1^{i+1},c_2^{i+1}}_{r_1^{i+1}}$), we get that $|B(\bigcup_{1\leq \ell \leq i} \mathsf{Area}(\ell) \cup \mathsf{Area}(i+1)|\leq |\mathsf{Area}^{c_1^{i+1}}|+ |\mathsf{Area}^{c_2^{i+1}}|+| \mathsf{Area}^{c_1^{i+1},c_2^{i+1}}_{r_2^{i+1}}|\leq 5\sqrt{n}$. So Condition \ref{dcon4} is satisfied..

Therefore, we overall get that $(\mathsf{Area}(i))_{1\leq i\leq k}$ is a nice decomposition of $G$, so $(c_1^i,c_2^i,r_1^i,r_2^i)_{1\leq i\leq k}$ is a nice RCL-cover of $G$.      
\end{proof}




\section{Data Structure and Preprocessing}

We now aim to construct our algorithm. First, we describe the data structure we work with (see Figure \ref{fi:DS}). Every vertex $v_{i,j}$ is an object. In addition, we have two arrays of size $c_{max}+2$, called $\mathsf{ColumnsArray}$ and $\mathsf{NiceColumnsArray}$. For every $0\leq i\leq c_{max}+1$, $\mathsf{ColumnsArray}[i]$ is an object, representing the $i$-th column of $H$. In $\mathsf{NiceColumnsArray}$ we store, throughout the computation of our algorithms, the ``nice columns pairs", as explained in Section \ref{section nice C and R}. Assume that we found $(c_1^i,c_2^i)_{1\leq i\leq k}$, pairs of nice columns through the computation of the algorithms. Observe that $k\leq c_{max}$. Then, for every $1\leq i\leq k$, $\mathsf{NiceColumnsArray}[i]$ represents the nice columns pair $(c_1^i,c_2^i)$. Every such $\mathsf{NiceColumnsArray}[i]$ is an object, storing the pair $(c_1^i,c_2^i)$, and also the set of vertices ``between" column $\mathsf{Area}_{c_1^i}$ and column $\mathsf{Area}_{c_2^i}$, that is, the set of vertices $\mathsf{Area}^{c_1^i,c_2^i}$. This set of vertices is given by a list, sorting the vertices of $\mathsf{Area}^{c_1^i,c_2^i}$ by their row number lexicographically. We call such a list an {\em SRLV} of $\mathsf{Area}^{c_1^i,c_2^i}$ (will be defined later). In addition, we make sure that the cell after the $k$-th pair of columns in $\mathsf{NiceColumnsArray}$, that is, $\mathsf{NiceColumnsArray}[k+1]$, stores $\mathsf{NULL}$ in its $c_1^{k+1}$, in order to mark that it is the first unused cell in $\mathsf{NiceColumnsArray}$.  

Now, we ``connect" each $\mathsf{ColumnsArray}[j]$, representing the $j$-th column of $H$, to the pair $(c_1^{i_j},c_2^{i_j})$, represented by $\mathsf{NiceColumnsArray}[i_j]$, that the column $\mathsf{Area}^j$ belongs to, that is, the pair such that $c_1^{i_j}<j\leq c_2^{i_j}$. We prove that the data structure we described can be computed in $\OO(n)$ time. We suppose that at the beginning of the computation, each vertex $v_{i,j}$ has a pointer to its corresponding column, that is, a pointer to $\mathsf{ColumnsArray}[j]$, and that we have $\mathsf{ColumnsArray}$ and $\mathsf{NiceColumnsArray}$ with $\mathsf{NULL}$ for all the ``values" we described so far. Indeed, observe that this can clearly be done in $\OO(n)$ time.      


%    Each Each $\mathsf{ColumnsArray}[i]$ pair of nice columns $(c_1^i,c_2^i)$    that we find . Assume that we found $0\leq i\leq n+1$  We assume that we have an ``array of columns" $\mathsf{ColumnsArray}$ with size $n+2$, such that every $\mathsf{ColumnsArray}[i]$ is an object. This array's role is to connect every column to its ``nice column area", which the algorithm finds during the computation of the nice RCL-cover. For these ``nice column area"  we have an ``array of nice columns" with size $n+2$, where the algorithm save the information about the pairs of nice columns it computes. We assume that every vertex $v_{i,j}$ is also an objects, and has a pointer to its column in $\mathsf{ColumnsArray}$, that is $\mathsf{ColumnsArray}[j]$. Later we add more information about the data structure. Observe that given a graph $G=(V,E)$ such  a data structure can be in $\OO(n)$ running time.


\begin{figure}[t!]
\centering
\includegraphics[width=0.75\textwidth, page=7]{figures/fig.pdf}
\caption{Illustration of the data structure. The vertex $v_{i,j}$ has a pointer to its corresponding column, $\mathsf{ColumnsArray}[j]$. The object $\mathsf{ColumnsArray}[j]$ represents column $\mathsf{Area}^j$, has a pointer to its corresponding nice columns pair, $(c_1^{t(j)},c_2^{t(j)})$, represented by $\mathsf{NiceColumnsArray}[t(j)]$, that is, the pair $(c_1^{t(j)},c_2^{t(j)})$ such that $c_1^{t(j)}<j\leq c_2^{t(j)}$. In addition, $\mathsf{NiceColumnsArray}[t(j)]$ has a pointer to an SRLV of $\mathsf{Area}^{c_1^{t(j)},c_2^{t(j)}}$. The first cell that is unused in $\mathsf{NiceColumnsArray}$ has the value $\mathsf{NULL}$ (in its $c_1^{k+1}$).}\label{fi:DS}
\end{figure}
      
%\begin{definition}[{\bf Rectangle-Columns-Lined-Up Cover}]\label{def:RCL} 
%Let $G=(V,E)$ be a connected grid graph and $H=(V',E')$. A sequence of quadruplets $(c_1^i,c_2^i,r_1^i,r_2^i)_{1\leq i\leq k}$ is a {\em rectangle-columns-lined-up cover (RCL-cover)} if the following conditions are satisfied.
%\begin{itemize}
%\item For every $1\leq i\leq k$, $c_2^i>c_1^i$ and $r_2^i>r_1^i$.
%\item For every $1\leq i<j\leq k$, if $c_1^i=c_1^j$ then $c_2^i=c_2^j$ and $r_1^j\geq r_2^i$. Otherwise $c_1^j\geq c_2^i$.
%\item There exist $1\leq i_1<i_2<\ldots <i_\ell \leq k$ such that $c_1^{i_1}=0$, $c_2^{i_\ell}=n+1$ and for every $1\leq j<\ell$ it follows that $c_1^{i_{j+1}}=c_2^{i_j}$.
%\item For every $1\leq i\leq k$ there exist $\ell \leq i\leq j$ such that $c_1^\ell=c_1^j=c_1^i$, $r_1^\ell=0, r_2^j=n+1$ and for every $\ell \leq m< j$ it follows that $r_1^{m+1}=r_2^m$.
  

%\end{itemize}    
%\end{definition}


%\begin{definition}[{\bf Nice Decomposition}]\label{def:niceDe} 
%Let $G=(V,E)$ be a connected grid graph. A {\em nice decomposition} of $G$ is a sequence of subsets of $V$ $(U_i)_{1\leq i\leq k}$ such that the following conditions are satisfied.
%\begin{enumerate}
%\item For every $v\in V(G)$ there exists $i$ such that $v\in U_i$. \label{dcon1}
%\item For every $1\leq i,j \leq k, i\neq j$ it follows that $U_i \cap U_j=\emptyset$. \label{dcon2}
%\item For every $1\leq i \leq k$ it follows that $\sqrt{n}\leq |U_i|\leq 5\sqrt{n}$. \label{dcon3}
%\item For every $1\leq i \leq k$ it follows that $|B(\bigcup_{1\leq \ell \leq i}U_\ell)|\leq 5\sqrt{n}$. \label{dcon4}
%\end{enumerate}

%\end{definition}

%\begin{definition}[{\bf Nice RCL-cover}]\label{def:niceDe} 
%Let $G=(V,E)$ be a connected grid graph. Let $(c_1^i,c_2^i,r_1^i,r_2^i)_{1\leq i\leq k}$ be an RCL-cover. If $(\mathsf{Area}^{c_1^i,c_2^i}_{r_1^i,r_2^i})_{1\leq i\leq k}$ is a nice decomposition of $G$, then $(c_1^i,c_2^i,r_1^i,r_2^i)_{1\leq i\leq k}$ is a {\em nice RCL-cover} of $G$.    
%\end{definition}





Recall that, our algorithm uses some lists of the vertices of $G$ sorted in a specific form. We denote by {\em SCLV} a list of vertices of $G$ sorted by their number of their column. Similarly, we denote by {\em SRLV} a list of vertices of $G$ sorted first by their number of row. We define these terms in the next definitions.   


\begin{definition} [{\bf SCLV}] Let $G=(V,E)$ be a grid graph. Then, a {\em sorted-by-columns list of the vertices ($\mathsf{SCLV}$)} of $G$ is a list of vertices in $V$ sorted by their number of column. That is, the vertices are sorted lexicographically, where the key of a vertex $u_{i,j}$ is $(j)$. 
\end{definition}

\begin{definition} [{\bf SRLV}] Let $G=(V,E)$ be a grid graph. Then, a {\em sorted-by-rows list of vertices ($\mathsf{SRLV}$)} of $G$ is a list of the vertices in $V$ sorted by their number of row. That is, the vertices are sorted lexicographically, where the key of a vertex $u_{i,j}$ is $(i)$. 
\end{definition}

%We assume that every vertex in SCLV has a pointer to the same vertex in SRLV and vice versa.

%Now, we present a simple algorithm that computes SCLV in $\OO(n)$ time, denoted as \ref{alg:SCLV}. The algorithm creates $n$ lists $L(i)$, one for each row. Then, it adds every vertex $v_{i,j}$ to $L(i)$. After that, the algorithm creats $n$ more lists $C(j)$, one for each column. Then, by iterating from $L(1)$ to $L(n)$ it adds every vertex $v_{i,j}\in L(i)$ to $C(j)$. Observe that after this step, we have that each $C(j)$ contains all the vertices that are located in the $j$-th column sorted by row. Then, the algorithm merges the $C(j)$ lists, and we get the SCLV of $G$. In Lemma \ref{lem:SCLV}, we prove the correctness and analyze the running time of the algorithm.    

Observe that an $\mathsf{SCLV}$ and an $\mathsf{SRLV}$ can be computed in $\OO(n)$ (for example using bucket sort). We state this in the next observation. 

\begin{observation}\label{lem:SCLV}
There exists an algorithm that, given a grid graph $G=(V,E)$, computes an $\mathsf{SCLV}$ and an $\mathsf{SRLV}$ of $G$ with running time $\OO(n)$.
\end{observation}



%\begin{algorithm}
 %   \SetKwInOut{Input}{Input}
    %\SetKwInOut{Output}{Output}
	%\medskip
   % {\textbf{function} $\mathsf{SCLV}$}$(\langle G=(V,E)\rangle)$\;
	%	Create $n$ empty sets, $L(i)$ for every $1\leq i\leq n$ \;
		%\For{every $v_{i,j}\in V$} {add $v_{i,j}$ to $L(i)$ \;}
		%\label{alg:SCLV1}
		%Create $n$ empty lists, $C(i)$ for every $1\leq i\leq n$ \;
		%\For{ $1\leq i\leq n$} 
	%	{
	%	\For{every $v_{i,j}\in L(i)$} {add $v_{i,j}$ to $C(j)$ \;}
	%	}
	%	\label{alg:SCLV9}
		
	%	Create an empty list $\mathsf{SCLV}$ \;
  %  \For{$1\leq i\leq n$} 
	%	{
	%	\While{$C(i)\neq \mathsf{null}$}
	%	{
	%	Add $C(i)$ to $\mathsf{SCLV}$\; 
	%	$C(i)\gets C(i).Next$\;
	%	}
	%	}
	%	\label{alg:SCLV3}
	%	Return $\mathsf{SCLV}$ \; \label{alg:SCLV2}
	
%    \caption{$\mathsf{SCLV}$}
%    \label{alg:SCLV}
%\end{algorithm}


%\begin{proof}
%We show that Algorithm \ref{alg:SCLV} finds SCLV. Observe that after Line \ref{alg:SCLV1}, set $L(i)$, for all $1\leq i\leq n$, contains exactly all the vertices that located at the $i$-th row.
%After Line \ref{alg:SCLV9}, each list $C(i)$, for all $1\leq i\leq n$, has all the vertices in column $i$ and only them, ordered by the number of row.  
%Therefore, after Line \ref{alg:SCLV3}, $\mathsf{SCLV}$ is an ordered by the number of column, merge of the lists $C(i)$ for $1\leq i\leq n$, we get that: if a vertex $v_{i,j}$ appears before $u_{i',j}$ in $\mathsf{SCLV}$, then $i\leq i'$.
%In conclusion, we get that Algorithm \ref{alg:SCLV} returns a list of the vertices in $V$ sorted first by their number of column, and second by their number of row. 
%Observe that this algorithm runs in $\OO(n)$ time. 
%A similar algorithm exists for getting SRLV with the obvious (symmetric) changes.     
%\end{proof}

In some case, we need a sorted list of a subset of $V$, for example, of some $\mathsf{Area}^{c_1,c_2}\subseteq V$. Then, when we refer to an $\mathsf{SRLV}$ of $\mathsf{Area}^{c_1,c_2}$, we refer a sorted list of the vertices of $\mathsf{Area}^{c_1,c_2}$ sorted by their number of row. 


%\begin{algorithm}
 %   \SetKwInOut{Input}{Input}
  %  \SetKwInOut{Output}{Output}
	%\medskip
   % {\textbf{function} $\mathsf{FindNiceColumns}$}$(\langle \mathsf{SCLV}\rangle)$\;
		
	%	Create an array $\mathsf{NiceColumnLocation}$ with $n+1$ cells\; 
		%$\mathsf{VerLeft}\gets n$ \;
		%$\mathsf{CurrentAreaCounter} \gets 0$\;
		%$\mathsf{CurrentNiceColumn}\gets 0$\;
		%$\mathsf{CurrentColumn}\gets 0$\;
		%$\mathsf{CurrentColumnCounter}\gets 0$\;
		%$\mathsf{NiceColumnLocation}[1].Start=0$\;
		
		%\While{True}
		%{
		
		%\While {$\mathsf{CurrentAreaCounter}<\sqrt{n}$}
			%{
			%$\mathsf{CurrentAreaCounter}\gets \mathsf{CurrentAreaCounter}+1$\;
			%\If{$\mathsf{SCLV}.Column \neq \mathsf{CurrentColumn}$}
			%{
				%$\mathsf{CurrentColumn}\gets \mathsf{SCLV}.Column$\;
				%$\mathsf{CurrentColumnCounter}\gets 0$\;
			%}
			%$\mathsf{CurrentColumnCounter}\gets \mathsf{CurrentColumnCounter}+1$\;
			%$\mathsf{SCLV}.NiceColumn=\mathsf{CurrentNiceColumn}$\;
			%$\mathsf{VerLeft}\gets \mathsf{VerLeft}-1$ \;
			%$\mathsf{SCLV} \gets \mathsf{SCLV}.Next$\;
			%}
				
		%\While {$\mathsf{SCLV}.Column \neq \mathsf{CurrentColumn}$}
		%{
		%	$\mathsf{CurrentColumnCounter}\gets \mathsf{CurrentColumnCounter}+1$\;
			%$\mathsf{SCLV}.NiceColumn=\mathsf{CurrentNiceColumn}$\;
			%$\mathsf{VerLeft}\gets \mathsf{VerLeft}-1$ \;
			%$\mathsf{SCLV} \gets \mathsf{SCLV}.Next$\;
			%$\mathsf{CurrentAreaCounter}\gets \mathsf{CurrentAreaCounter}+1$\;
		%}
		
		%\While {$\mathsf{CurrentColumnCounter} >\sqrt{n}$}
		%{
		%$\mathsf{CurrentColumn}\gets \mathsf{SCLV}.Column$\;
		%$\mathsf{CurrentColumnCounter}\gets 0$\;
		
		%\While {$\mathsf{SCLV}.Column \neq \mathsf{CurrentColumn}$}
		%{
			%$\mathsf{CurrentColumnCounter}\gets \mathsf{CurrentColumnCounter}+1$\;
			%$\mathsf{SCLV}.NiceColumn=\mathsf{CurrentNiceColumn}$\;
			%$\mathsf{CurrentAreaCounter}\gets \mathsf{CurrentAreaCounter}+1$\;
			%$\mathsf{VerLeft}\gets \mathsf{VerLeft}-1$ \;
			%$\mathsf{SCLV} \gets \mathsf{SCLV}.Next$\;
		%}
		%}
		%\If {$\mathsf{VerLeft}<{\sqrt{n}}$}
		%{
			%$\mathsf{NiceColumnLocation}[\mathsf{CurrentNiceColumn}].Finish=n+1$\;
			%$\mathsf{NiceColumnLocation}[\mathsf{CurrentNiceColumn}].NumOfVer=\mathsf{VerLeft}+\mathsf{CurrentAreaCounter}$\;
			%\While {$\mathsf{SCLV}\neq$ Null}
			%{	
				%$\mathsf{SCLV}.NiceColumn=\mathsf{CurrentNiceColumn}$\;
				%$\mathsf{SCLV} \gets \mathsf{SCLV}.Next$\;
			%}
			%$\mathsf{NiceColumnLocation}[0]=\mathsf{CurrentNiceColumn}$ \;
			%Return $\mathsf{NiceColumnLocation}$ \;
		%}
		%$\mathsf{NiceColumnLocation}[\mathsf{CurrentNiceColumn}].Finish=\mathsf{CurrentColumn}$\;
		%$\mathsf{CurrentNiceColumn}\gets \mathsf{CurrentNiceColumn}+1$\;
		%$\mathsf{NiceColumnLocation}[\mathsf{CurrentNiceColumn}].Start=\mathsf{CurrentColumn}$\;
		%$\mathsf{NiceColumnLocation}[\mathsf{CurrentNiceColumn}].NumOfVer=\mathsf{CurrentAreaCounter}$\;
		%$\mathsf{CurrentAreaCounter} \gets 0$\;
	%$\mathsf{CurrentColumnCounter}\gets 0$\;
		%}
		
		
   % \caption{$\mathsf{NiceColumnsUpdater}$}
   % \label{alg:SCLV}
%\end{algorithm}


%\begin{algorithm}
 %   \SetKwInOut{Input}{Input}
  %  \SetKwInOut{Output}{Output}
	%\medskip
   % {\textbf{function} $\mathsf{SRLV}$}$(\langle G=(V,E), \mathsf{NiceColumnLocation} \rangle)$\;
		
		%Create $n$ empty sets $R[i]$ for every $1\leq i\leq n$\;
		%\For {every $v_{i,j}\in V$}
		%{
		%$R[i]\gets v_{i,j}$\;
		%}
		%Create $\mathsf{NiceColumnLocation}[0]-1$ empty Lists $\mathsf{AreaByRow^{i}}$ for every $1\leq i\leq \mathsf{NiceColumnLocation}[0]-1$\;
		%\For {$i=1$ to $n$}
		%{
		%\For {every $v_{i,j}\in R[i]$}
		%{
		%	$k\gets v_{i,j}.NiceColumn$\;
			%Add $v_{i,j}$ to $\mathsf{AreaByRow^{k}}$\;
		%}
		%}
		%Return $\{ \mathsf{AreaByRow^{i}} \}_{i=1}^{\mathsf{NiceColumnLocation}[0]-1}$\;
		
	
    %\caption{$\mathsf{AreasByRow}$}
    %\label{alg:NextNiceRow}
%\end{algorithm}


%\begin{algorithm}
 %   \SetKwInOut{Input}{Input}
  %  \SetKwInOut{Output}{Output}
	%\medskip
   % {\textbf{function} $\mathsf{AreaPrinter}$}$(\langle G=(V,E), \mathsf{Area}, c_1, c_2, \mathsf{NumOfVer}  \rangle)$\;
		
		
		%$\mathsf{VerLeft}\gets \mathsf{NumOfVer}$ \;
		%$\mathsf{CurrentAreaCounter} \gets 0$\;
		%$\mathsf{CurrentNiceRow}\gets 0$\;
		%$\mathsf{CurrentRow}\gets 0$\;
		%$r_1\gets 0$\;
	
	%\While{$\mathsf{VerLeft}>0$}
	%{
	%\While {$\mathsf{CurrentAreaCounter}<\sqrt{n}$}
	%{
		%$\mathsf{CurrentAreaCounter} \gets \mathsf{CurrentAreaCounter}+1$\;
		%$\mathsf{VerLeft}\gets \mathsf{VerLeft}-1$\;
		%\If{$\mathsf{CurrentRow}\neq \mathsf{Area}.Row$}
		%{
		%	$\mathsf{CurrentRow}= \mathsf{Area}.Row$\;
		%}
		%$\mathsf{Area}\gets \mathsf{Area}.Next$\;
	%}
	%\While{$\mathsf{CurrentRow}= \mathsf{Area}.Row$}
	%{
	%$\mathsf{Area}\gets \mathsf{Area}.Next$\;
	%$\mathsf{VerLeft}\gets \mathsf{VerLeft}-1$\;
	%}
	%\If {$\mathsf{VerLeft}<\sqrt{n}$}
	%{
	%	Print$(c_1,c_2,r_1,n+1)$\;
	%	Return \;
	%}
	%Print$(c_1,c_2,r_1,\mathsf{CurrentRow})$\;
	%$r_1\gets \mathsf{CurrentRow}$\;
	%$\mathsf{CurrentRow}\gets \mathsf{Area}.Row$\;
	%$\mathsf{CurrentAreaCounter} \gets 0$\;
	
%	}
	%Return\;
   % \caption{$\mathsf{AreaCoverPrinter}$}
    %\label{alg:NextNiceRow}
%\end{algorithm}




%\begin{algorithm}
 %   \SetKwInOut{Input}{Input}
  %  \SetKwInOut{Output}{Output}
	%\medskip
  %  {\textbf{function} $\mathsf{NiceRCLCoverPrinter}$}$(\langle G=(V,E), \mathsf{NiceColumnLocation},\{ \mathsf{AreaByRow^{i}} \}_{i=1}^{\ell} \rangle)$\;
		
%	\For{$i=1$ to $\mathsf{NiceColumnLocation}-1$}
	%{
	%$\mathsf{Area}\gets \mathsf{AreaByRow^{i}}$\;
	%$c_1\gets \mathsf{NiceColumnLocation}[i].Start$\;
	%$c_2\gets \mathsf{NiceColumnLocation}[i].Finish$\;
	%$\mathsf{NumOfVer}\gets \mathsf{NiceColumnLocation}[i].NumOfVer$\;
	
		%$\mathsf{AreaPrinter} (G=(V,E), \mathsf{Area},c_1,c_2,\mathsf{NumOfVer})$\;
	%}
	
	
%\caption{$\mathsf{NiceRCLCoverPrinter}$}
%    \label{alg:NextNiceRow}
%\end{algorithm}


\section{Algorithm}

In this section, we are ready to present our algorithm that computes a nice RCL-cover of $G$ with running time $\OO(n)$. We first state main theorem of this paper, which we will prove later (in this section):

\begin{theorem}\label{lem:algo exists}
There exists an algorithm that, given a connected grid graph $G=(V,E)$ with $n$ vertices, runs in $\OO(n)$ time and computes a nice RCL-cover of $G$.  
\end{theorem}

Towards the proof of Theorem \ref{lem:algo exists}, we describe several algorithms to be used later as subprocedures.

In Algorithm \ref{alg:NextNiceColumn}, we find a next nice column by iterating over the vertices of the graph $G$ in an $\mathsf{SCLV}$. The algorithm takes as input a pointer to an $\mathsf{SCLV}$, denoted by $\mathsf{SCLVpointer}$. We assume that the $\mathsf{SCLVpointer}$ points to the first vertex of a column $\mathsf{Area}^{i+1}$ where $\mathsf{Area}^{i,c_{max}+1}\geq \sqrt{n}$. The algorithm counts the vertices while iterating over the vertices in $\mathsf{SCLV}$ until it reaches $\sqrt{n}$ vertices. Then, the algorithm finds the first column $\mathsf{Area}^{j}$ that contains $\sqrt{n}$ or less vertices. The existence of such a column is guaranteed as shown in Lemma \ref{lem:Nice column}. After that, the algorithm checks if the number of the rest of the vertices in the $\mathsf{SCLV}$ is larger than $\sqrt{n}$. If it is, then the algorithm returns $\mathsf{Area}^{j}$ as the next nice column. Otherwise, it returns the $(c_{max}+1)$-th column. Observe that, in either case, the algorithm returns an almost nice column with respect to $\mathsf{Area}^{i}$. In the case where the algorithm returns $\mathsf{Area}^{j}$, we also make sure that $\mathsf{SCLVpointer}$ points to the first vertex of column $\mathsf{Area}^{j+1}$, so we can use the algorithm to find the next nice column iteratively.     


\begin{algorithm}[!t]
    \SetKwInOut{Input}{Input}
    \SetKwInOut{Output}{Output}
	\medskip
    {\textbf{function} $\mathsf{NextNiceColumn}$}$(\langle \mathsf{SCLVpointer}\rangle)$\;
		
    	$\mathsf{Area}\gets 1$\;
			$\mathsf{AreaInColumn}\gets 1$\;
			$\mathsf{CurrentCoulmn}\gets \mathsf{SCLVpointer.column}$\;
			 \While{$\mathsf{Area}<\sqrt{n}$} 
			{
				 \label{algo3:line5} $\mathsf{Area}\gets \mathsf{Area}+1$\;
				\If{$\mathsf{SCLVpointer.Next.column}=\mathsf{CurrentCoulmn}$}
				{$\mathsf{AreaInColumn}\gets \mathsf{AreaInColumn}+1$\;}
				\Else{
				$\mathsf{CurrentCoulmn}\gets \mathsf{SCLVpointer.Next.column}$\;
				$\mathsf{AreaInColumn}\gets 1$\;
				}
				$\mathsf{SCLVpointer} \gets \mathsf{SCLVpointer.Next}$\;
			}
			\While {$\mathsf{SCLVpointer.Next.column}= \mathsf{CurrentCoulmn}$} 
			{
			\label{algo3:line16} $\mathsf{SCLVpointer} \gets \mathsf{SCLVpointer.Next}$\;
			$\mathsf{AreaInColumn}\gets \mathsf{AreaInColumn}+1$\;
			}
			 \While {$\mathsf{AreaInColumn}>\sqrt{n}$}  
			{
			\label{algo3:line20} $\mathsf{SCLVpointer} \gets \mathsf{SCLVpointer.Next}$\; 
		\label{algo3:line21}	$\mathsf{CurrentCoulmn}\gets \mathsf{SCLVpointer.column}$\;
			$\mathsf{AreaInColumn}\gets 1$\;
			\While {$\mathsf{SCLVpointer.Next.column}= \mathsf{CurrentCoulmn}$}
			{
			$\mathsf{SCLVpointer} \gets \mathsf{SCLVpointer.Next}$\;
			$\mathsf{AreaInColumn}\gets \mathsf{AreaInColumn}+1$\; \label{algo3:line26} 
			}
			}
			$\mathsf{RestOfArea}\gets 0$\;\label{algo3:line29}
			$\mathsf{SCLVpointerTemp}\gets \mathsf{SCLVpointer}$\; \label{algo3:while3}
		\While{$\mathsf{RestOfArea}< \sqrt{n}$ and $\mathsf{SCLVpointerTemp.Next}\neq \mathsf{Null}$ } 
			{
				\label{algo3:line31} $\mathsf{SCLVpointerTemp}\gets \mathsf{SCLVpointerTemp.Next}$\;
			$\mathsf{RestOfArea}\gets \mathsf{RestOfArea} +1$\;
			}
			\If {$\mathsf{RestOfArea}=\sqrt{n}$} 
			 \Return $\mathsf{CurrentCoulmn}$\; 
			{\label{algo3:line36} $\mathsf{SCLVpointer} \gets \mathsf{SCLVpointer.Next}$\;}
			 \Else {\Return $c_{max}+1$\;} 
			
				\label{algo3:line39}
			
	
    \caption{$\mathsf{NextNiceColumn}$}
    \label{alg:NextNiceColumn}
\end{algorithm}


In the following lemma, we prove the correctness of Algorithm \ref{alg:NextNiceColumn} and analyze its running time.

\begin{lemma} \label{lem:colum}
Let $G=(V,E)$ be a connected grid graph with $n$ vertices, and let $0\leq i<c_{max}+1$ such that $\mathsf{Area}^{i,c_{max}+1}\geq \sqrt{n}$. Let $\mathsf{SCLVpointer}$ be a pointer to an $\mathsf{SCLV}$ of $G$, and assume that $\mathsf{SCLVpointer}$ points to the first vertex of column $\mathsf{Area}^{i+1}$. Then, Algorithm \ref{alg:NextNiceColumn} takes $\mathsf{SCLVpointer}$ as input, and returns $i<j\leq c_{max}+1$ such that the following conditions are satisfied.
\begin{enumerate}
\item $\mathsf{Area}^{j}$ is an almost nice column with respect to $\mathsf{Area}^{i}$.
\item If $j\neq c_{max}+1$, then $\mathsf{Area}^{j,c_{max}+1}>\sqrt{n}$.
\item If $j\neq c_{max}+1$, then $\mathsf{SCLVpointer}$ points to the first vertex of column $\mathsf{Area}^{j+1}$ at the end of the algorithm.    
\end {enumerate} 
In addition, the algorithm runs in time $\OO(|\mathsf{Area}^{i,j}|)$.      
\end{lemma}

\begin{proof}
Since $\mathsf{Area}^{i,c_{max}+1}\geq \sqrt{n}$, by Lemma \ref{lem:Nice column}, we get that there exists $i<j'\leq c_{max}+1$ such that $\mathsf{Area}^{j'}$ is a nice column with respect to $\mathsf{Area}^{i}$. Let $j$ be the smallest such $j'$. From Definition \ref{def:Nice column}, we get that $\mathsf{Area}^{i,j}\geq \sqrt{n}$, so the number of vertices in an $\mathsf{SCLV}$ of $G$ from the first vertex of column $\mathsf{Area}^{i+1}$ to the last vertex of column $\mathsf{Area}^{j}$ is at least $\sqrt{n}$. Therefore, there exists $u_{k,\ell}$ such that $i<\ell\leq j$ and the number of vertices in the $\mathsf{SCLV}$ of $G$ from the first vertex of column $\mathsf{Area}^{i+1}$ to $u_{k,\ell}$ is exactly $\sqrt{n}$. Therefore, when we are in the while loop in Line \ref{algo3:line5} in the iteration where $\mathsf{SCLVPointer}$ points to $u_{k,\ell}$, we have that $\mathsf{Area}=\sqrt{n}$; so, the algorithm proceeds to Line \ref{algo3:line16}. Now, from Definition \ref{def:Nice column} and from the minimality of $j$, we get that $\mathsf{Area}^{j}$ is the first column with at most $\sqrt{n}$ vertices after column $\mathsf{Area}^{\ell}$. Therefore, in the iteration of the while loop in Line \ref{algo3:line20}, when $\mathsf{SCLVPointer}$ points to the last vertex in column $\mathsf{Area}^{j}$, the condition $\mathsf{AreaInColumn}\leq \sqrt{n}$ is satisfied for the first time, so the algorithm proceeds to Line \ref{algo3:line29}. At this point, observe that $\mathsf{CurrentColumn}=j$ and $\mathsf{SCLVPointer}$ points to the last vertex in column $\mathsf{Area}^{j}$. Notice that none of $\mathsf{CurrentColumn}=j$ and $\mathsf{SCLVPointer}$ changes until the end of the algorithm from this point. Now, observe that if $\mathsf{Area}^{j,c_{max}+1}\geq \sqrt{n}$, then after $\sqrt{n}$ iterations, the while loop in Line \ref{algo3:line31} ends when $\mathsf{RestOfArea}=\sqrt{n}$. In this case, the algorithm returns $\mathsf{CurrentColumn}=j$ in Line \ref{algo3:line36}, and the conditions are satisfied. 

If $\mathsf{Area}^{j,c_{max}+1}< \sqrt{n}$, then after less than $\sqrt{n}$ iterations, the while loop in Line \ref{algo3:line31} ends and $\mathsf{RestOfArea}<\sqrt{n}$. In this case, the algorithm returns $c_{max}+1$ in Line \ref{algo3:line39}. By Observation \ref{obs:n+1 is almost} we get that $\mathsf{Area}^{c_{max}+1}$ is an almost nice column with respect to $\mathsf{Area}^{i}$, so the conditions are satisfied.

As for the running time, it is easy to see that the $\mathsf{SCLVPointer}$ pointer moves only forward in the $\mathsf{SCLV}$, therefore the total number of iterations in the while loops in Lines \ref{algo3:line5}, \ref{algo3:line16} and \ref{algo3:line20} is $(|\mathsf{Area}^{i,j}|)$, and the running time of every iteration is bounded by a constant. The number of iterations of the while loop in Line \ref{algo3:line31} is bounded by $\sqrt{n}$, and the running time of every iteration is bounded by a constant. The running time of the rest of the algorithm is also bounded by a constant. Therefore, the total running time of the algorithm is $\OO(|\mathsf{Area}^{i,j}|)+\OO (\sqrt{n})$, and since $|\mathsf{Area}^{i,j}|\geq \sqrt{n}$ we get that the running time is $\OO(|\mathsf{Area}^{i,j}|)$.                     
\end{proof}



In Algorithm \ref{alg:NextNiceRow}, we find the ``next nice row" by iterating over the vertices of the graph $G$ in an $\mathsf{SRLV}$ of $\mathsf{Area}^{c_1,c_2}$, where $\mathsf{Area}^{c_2}$ is an almost nice column with respect to $\mathsf{Area}^{c_1}$. The algorithm gets as input a pointer $\mathsf{SRLVpointer}$ to an $\mathsf{SRLV}$ of $\mathsf{Area}^{c_1,c_2}$. We assume that $\mathsf{SRLVpointer}$ points to the first vertex of a row $\mathsf{Area}^{c_1,c_2}_{k+1}$ where $\mathsf{Area}^{c_1,c_2}_{k,r_{max}+1}\geq \sqrt{n}$. The algorithm counts the vertices while iterating through the vertices in the $\mathsf{SRLV}$ until it reaches $\sqrt{n}$ vertices. Assume that $\mathsf{Area}^{c_1,c_2}_{\ell}$ is the row of the vertex to which $\mathsf{SRLVpointer}$ points at this step. Observe that $\mathsf{Area}^{c_1,c_2}_{\ell}$ is a nice row with respect to $\mathsf{Area}^{c_1,c_2}_{k}$. The existence of such a row is guaranteed as shown in Lemma \ref{lem:nice row}. Then, the algorithm iterates until $\mathsf{SRLVpointer}$ points to the first vertex of row $\mathsf{Area}^{c_1,c_2}_{\ell+1}$. After that, the algorithm checks if the number of the rest of the vertices in the $\mathsf{SRLV}$ is larger than $\sqrt{n}$. If it is, then the algorithm returns $\mathsf{Area}^{c_1,c_2}_{\ell}$ as the next nice row. Otherwise, it returns the $(n+1)$-th row. Observe that in either case the algorithm returns an almost nice row with respect to $\mathsf{Area}^{c_1,c_2}_{k}$. Moreover, in the case where the algorithm returns a row $\mathsf{Area}^{c_1,c_2}_{\ell}$ other than $\mathsf{Area}^{c_1,c_2}_{r_{max}+1}$, $\mathsf{SRLVpointer}$ points to the first vertex of row $\mathsf{Area}^{c_1,c_2}_{\ell+1}$, so we can use the algorithm to find the next nice row iteratively.     

%Next, Algorithm \ref{alg:NextNiceRow} is given $1\leq i<j\leq n+1$ such that $\mathsf{Area}^{j}$ is an almost nice column with respect to $\mathsf{Area}^{i}$ and a row $\mathsf{Area}^{i,j}_{k}$. The algorithm finds the next nice row by iterating the vertices of the graph in the $\mathsf{SRLV}$ of $\mathsf{Area}^{i,j}$. The existences of such a column is guaranteed as we show in Lemma \ref{lem:nice row}.     

\begin{algorithm}[!t]
    \SetKwInOut{Input}{Input}
    \SetKwInOut{Output}{Output}
	\medskip
    {\textbf{function} $\mathsf{NextNiceRow}$}$(\langle \mathsf{SRLVpointer}\rangle)$\;
		
    	$\mathsf{Area}\gets 1$\;
			$\mathsf{AreaInRow}\gets 1$\;
			$\mathsf{CurrentRow}\gets \mathsf{SRLVpointer.row}$\;
			\While{$\mathsf{Area}<\sqrt{n}$} 
			{
				\label{algo4:line5} $\mathsf{Area}\gets \mathsf{Area}+1$\;
				\If{$\mathsf{SRLVpointer.Next.row}=\mathsf{CurrentRow}$}
				{$\mathsf{AreaInRow}\gets \mathsf{AreaInRow}+1$\;}
				\Else{
				$\mathsf{CurrentRow}\gets \mathsf{SRLVpointer.Next.row}$\;
				$\mathsf{AreaInRow}\gets 1$\;
				}
				$\mathsf{SRLVpointer} \gets \mathsf{SRLVpointer.Next}$\;
			}
			\While {$\mathsf{SRLVpointer.Next.row}= \mathsf{CurrentRow}$}
			{
			\label{algo4:line16}
			$\mathsf{SRLVpointer} \gets \mathsf{SRLVpointer.Next}$\;
			}
			$\mathsf{RestOfArea}\gets 0$\;
			$\mathsf{SRLVpointerTemp}\gets \mathsf{SRLVpointer}$\; 
			\While{$\mathsf{RestOfArea}< \sqrt{n}$ And $\mathsf{SRLVpointerTemp.Next}\neq \mathsf{Null}$ }
			{
			\label{algo4:line21}$\mathsf{SRLVpointerTemp}\gets \mathsf{SRLVpointerTemp.Next}$\;
			$\mathsf{RestOfArea}\gets \mathsf{RestOfArea} +1$\;
			}
			\If {$\mathsf{RestOfArea}=\sqrt{n}$} 
			{\Return $\mathsf{CurrentRow}$\;
			\label{algo4:line26}$\mathsf{SRLVpointer} \gets \mathsf{SRLVpointer.Next}$\;}
				\Else {\label{algo4:line30} \Return $r_{max}+1$\;}
			
			
			
	
    \caption{$\mathsf{NextNiceRow}$}
    \label{alg:NextNiceRow}
\end{algorithm}

In the following lemma, we prove the correctness of Algorithm \ref{alg:NextNiceRow} and analyze its running time.

\begin{lemma} \label{lem:row}
Let $G=(V,E)$ be a connected grid graph with $n$ vertices, and let $1\leq i<j\leq c_{max}+1$ such that $\mathsf{Area}^{j}$ is an almost nice column with respect to $\mathsf{Area}^{i}$. Let $0\leq k<r_{max}+1$ such that $\mathsf{Area}^{i,j}_{k,r_{max}+1}\geq \sqrt{n}$. Let $\mathsf{SRLVpointer}$ be a pointer of an $\mathsf{SRLV}$ of $\mathsf{Area}^{i,j}$ and assume that $\mathsf{SRLVpointer}$ points to the first vertex of the row $\mathsf{Area}^{i,j}_{k+1}$. Then, Algorithm \ref{alg:NextNiceRow} takes $\mathsf{SRLVpointer}$ as input and returns $k<p\leq r_{max}+1$ such that the following conditions are satisfied.
\begin{itemize}
\item $\mathsf{Area}^{i,j}_{p}$ is an almost nice row with respect to $\mathsf{Area}^{i,j}_{k}$.
\item If $p\neq r_{max}+1$, then $\mathsf{Area}^{i,j}_{p,r_{max}+1}>\sqrt{n}$.
\item If $p\neq r_{max}+1$, then $\mathsf{SRLVpointer}$ points to the first vertex of row $\mathsf{Area}^{i,j}_{p+1}$ at the end of the algorithm.    
\end{itemize}
Moreover, Algorithm \ref{alg:NextNiceRow} runs in time $\OO(|\mathsf{Area}^{i,j}_{k,p}|)$.      
\end{lemma}

%Now, observe that after the while loop we get that $\mathsf{SRLVpointer}$ points to the first vertex of row $\mathsf{Area}^{i,j}_{\ell+1}$.

\begin{proof}
Since $\mathsf{Area}^{i,j}_{k,r_{max}+1}\geq \sqrt{n}$, by Lemma \ref{lem:nice row}, we get that there exists $i<p'\leq r_{max}+1$ such that $\mathsf{Area}^{i,j}_{p'}$ is a nice row with respect to $\mathsf{Area}^{i,j}_{k}$. Let $p$ be the smallest such $p'$. From Definition \ref{def:Nice Row}, we get that $\mathsf{Area}^{i,j}_{k,p}\geq \sqrt{n}$. Therefore, there exists $u_{s,\ell}$ such that $i<\ell\leq j$, $k<s\leq p$ and the number of vertices in an $\mathsf{SRLV}$ of $\mathsf{Area}^{i,j}$ from the first vertex of row $\mathsf{Area}^{i,j}_{k+1}$ to $u_{s,\ell}$ is exactly $\sqrt{n}$. Therefore, in the while loop in Line \ref{algo4:line5}, in the iteration when $\mathsf{SRLVPointer}$ points to $u_{s,\ell}$, we get that $\mathsf{Area}=\sqrt{n}$, so the algorithm proceeds to Line \ref{algo4:line16}. Observe that, since $\mathsf{Area}^{j}$ is an almost nice column with respect to $\mathsf{Area}^{i}$, $\mathsf{Area}^{i,j}_{\ell}\leq 5\sqrt{n}$. Therefore, we get that $\ell$ is the minimal $p'$ such that $\mathsf{Area}^{i,j}_{\ell}$ is a nice row with respect to $\mathsf{Area}^{i,j}_{k}$, i.e., $p=\ell$. At this point, observe that $\mathsf{CurrentRow}=p$ and $\mathsf{SRLVPointer}$ points to the last vertex in row $\mathsf{Area}^{i,j}_{p}$. Notice that none of $\mathsf{CurrentRow}=p$ and $\mathsf{SRLVPointer}$ changes until the end of the algorithm from this point. Now, observe that if $\mathsf{Area}^{i,j}_{p,r_{max}+1}\geq \sqrt{n}$, then after $\sqrt{n}$ iterations, the while loop in Line \ref{algo4:line21} ends when $\mathsf{RestOfArea}=\sqrt{n}$. In this case, the algorithm returns $\mathsf{CurrentRow}=p$ in Line \ref{algo4:line26}, and the conditions are satisfied. 

If $\mathsf{Area}^{i,j}_{p,r_{max}+1}< \sqrt{n}$, then after less than $\sqrt{n}$ iterations the while loop in Line \ref{algo4:line21} ends when $\mathsf{RestOfArea}<\sqrt{n}$. In this case, the algorithm returns the $(r_{max}+1)$-th row in Line \ref{algo4:line30}. By Observation \ref{obs:n+1 is almost row}, we get that $\mathsf{Area}^{i,j}_{r_{max}+1}$ is an almost nice row with respect to $\mathsf{Area}^{i,j}_k$, so the conditions are satisfied.

As for the running time, it is easy to see that the $\mathsf{SRLVPointer}$ pointer moves only forward in the $\mathsf{SRLV}$ of $\mathsf{Area}^{i,j}$, therefore the total number of iterations in the while loops in Lines \ref{algo4:line5} and \ref{algo4:line16} is $(|\mathsf{Area}^{i,j}_{k,p}|)$, and the running time of every iteration is bounded by a constant. The number of iterations of the while loop in Line \ref{algo4:line21} is bounded by $\sqrt{n}$, and the running time of every iteration is bounded by a constant. The running time of the rest of the algorithm is also bounded by a constant. Therefore, the total running time of the algorithm is $\OO(|\mathsf{Area}^{i,j}_{k,p}|)+\OO (\sqrt{n})$, and since $|\mathsf{Area}^{i,j}_{k,p}|\geq \sqrt{n}$, we get that the running time is $\OO(|\mathsf{Area}^{i,j}_{k,p}|)$.             
\end{proof}




We now consider Algorithm \ref{alg:NiceColumnsUpdater}, which uses Algorithm \ref{alg:NextNiceColumn} in order to find a sequence of pairs $(c_1^i,c_2^i)_{1\leq i\leq k}$ of nice columns. It updates $\mathsf{NiceColumnsArray}$ accordingly and connects every vertex $v$ to its nice columns pair, i.e., the pair $(c_1^i,c_2^i)$ such that $v\in \mathsf{Area}^{c_1,c_2}$.

\begin{algorithm}[!t]
    \SetKwInOut{Input}{Input}
    \SetKwInOut{Output}{Output}
	\medskip
    {\textbf{function} $\mathsf{NiceColumnsUpdater}$}$(\langle G=(V,E) \rangle)$\;
			$\mathsf{SCLVpointer}\gets$ $\mathsf{SCLV}$ of $G$\;
			$i\gets 1$\;
			$\mathsf{currentColumn}\gets 0$\;
    	$c_1\gets 0$\;
			$c_2\gets \mathsf{NextNiceColumn}\langle \mathsf{SCLVpointer}\rangle$\;
			\label{algo5:line6}$\mathsf{NiceColumnsArray}[i].c_1\gets c_1$\;
			\label{algo5:line7}$\mathsf{NiceColumnsArray}[i].c_2\gets c_2$\;
			\label{algo5:line8}\While{$\mathsf{currentColumn}\leq c_2$}
			{
			\label{algo5:line9}	$\mathsf{currentColumn}\gets \mathsf{currentColumn}+1$\;
				$\mathsf{ColumnsArray}[\mathsf{currentColumn}].niceColumn\gets i$\;
			}
			\While {$c_2 \neq c_{max}+1$}
			{\label{algo5:line13}
			$i\gets i+1$\;
			$c_1\gets c_2$\;
			\label{algo5:line15}$c_2\gets \mathsf{NextNiceColumn}\langle \mathsf{SCLVpointer}\rangle$\;
			\label{algo5:line16}$\mathsf{NiceColumnsArray}[i].c_1\gets c_1$\;
			\label{algo5:line17}$\mathsf{NiceColumnsArray}[i].c_2\gets c_2$\;
			\label{algo5:line18}\While{$\mathsf{currentColumn}\leq c_2$}
			{
				\label{algo5:line19}$\mathsf{currentColumn}\gets \mathsf{currentColumn}+1$\;
				$\mathsf{ColumnsArray}[\mathsf{currentColumn}].niceColumn\gets i$\;
			}
			}
			$\mathsf{NiceColumnsArray}[i+1].c_1\gets Null$\;
			
			\label{algo5:line24}
	
			\Return \;
				
    \caption{$\mathsf{NiceColumnsUpdater}$}
    \label{alg:NiceColumnsUpdater}
\end{algorithm}


%---------------------------------------------------------------------------------------------------------------------------------------------------------
In the next lemma, we prove the correctness of Algorithm \ref{alg:NiceColumnsUpdater} and analyze its running time. 


\begin{lemma} \label{lem:columnUpdater}
Let $G=(V,E)$ be a connected grid graph with $n$ vertices. Then, Algorithm \ref{alg:NiceColumnsUpdater} takes $G=(V,E)$ as input, runs in time $\OO(n)$ and computes $(c_1^i,c_2^i)_{1\leq i\leq k}$ such that the following conditions are satisfied.
\begin{enumerate}
\item $c_1^1=0$ and $c_2^k=c_{max}+1$. \label{lem:ColumnUpdaterCon1}
\item For every $1\leq i\leq k$, $c_2^i$ is an almost nice column with respect to $c_2^i$. \label{lem:ColumnUpdaterCon2}
\item For every $1\leq i< k$, $c_2^i=c_1^{i+1}$. \label{lem:ColumnUpdaterCon3}
 \end{enumerate}
The algorithm updates $\mathsf{NiceColumnsArray}$ so that for every $1\leq i\leq k$, $\mathsf{NiceColumnsArray}[i].c_1$ $=c_1^i$,
$\mathsf{NiceColumnsArray}[i].c_2=c_2^i$ and $\mathsf{NiceColumnsArray}[k+1].c_1=NULL$. In addition, the algorithm updates $\mathsf{ColumnsArray}$ so that for every $1\leq i\leq n$, it follows that $\mathsf{ColumnsArray}[i]$ $.niceColumn=j$ where $\mathsf{NiceColumnsArray}[j].c_1<i\leq \mathsf{NiceColumnsArray}[j].c_2$. 
\end{lemma}

\begin{proof}
Observe that in Line \ref{algo5:line6}, Algorithm \ref{alg:NextNiceColumn} is given as input $\mathsf{SCLVpointer}$, where $\mathsf{SCLVpointer}$ is a pointer to the first vertex in an $\mathsf{SCLV}$ of $G$. Therefore, by Lemma \ref{lem:column}, Algorithm \ref{alg:NextNiceColumn} returns $0<p\leq n+1$ such that $\mathsf{Area}^{0,p}$ is an almost nice column with respect to $\mathsf{Area}^{0}$. So, the first pair that the algorithm computes is $(0,p)$. Therefore, the sequence of pairs the algorithm computes is not empty. Later, we show that this sequence is finite.

Let $(c_1^i,c_2^i)_{1\leq i\leq k}$ be a prefix of the sequence of pairs the algorithm computes. We show by induction that Condition \ref{lem:ColumnUpdaterCon2} is satisfied for every $1\leq i\leq k$. We argue that for every $1\leq i\leq k$, it follows that $\mathsf{Area}^{c_1^i}$ is an almost nice column with respect to $\mathsf{Area}^{c_2^i}$. Moreover, if $c_2^i\neq c_{max}+1$, then $\mathsf{Area}^{c_2,c_{max}+1}>\sqrt{n}$ and $\mathsf{SCLVpointer}$ points to the first vertex of column $\mathsf{Area}^{c_2^i+1}$ at the time the algorithm computes $(c_1^i,c_2^i)$. 

For $i=1$, we saw that Condition \ref{lem:ColumnUpdaterCon2} is satisfied. Now, if in Line \ref{algo5:line6} Algorithm \ref{alg:NextNiceColumn} returns $c_2^1< c_{max}+1$ then by Lemma \ref{lem:column} we get that $\mathsf{Area}^{c_2^1,c_{max}+1}>\sqrt{n}$ and $\mathsf{SCLVpointer}$ points to the first vertex of column $\mathsf{Area}^{c_2^1+1}$. Thus, we have proved the statement for $i=1$.

Now, let $1< i\leq k$. Observe that the algorithm computes $(c_1^i,c_2^i)$ in Line \ref{algo5:line16}. Therefore, because of the condition of the while loop in Line \ref{algo5:line13}, we get that $c_2^{i-1}\neq c_{max}+1$. So, by the inductive hypothesis, we get that $\mathsf{Area}^{c_2^{i-1},c_{max}+1}>\sqrt{n}$ and $\mathsf{SCLVpointer}$ points to the first vertex of column  $\mathsf{Area}^{c_2^{i-1}+1}$. Therefore, by Lemma \ref{lem:column}, we get that in Line \ref{algo5:line16}, Algorithm \ref{alg:NextNiceColumn} returns $c_2^{i-1}<c_2^i\leq c_{max}+1$ such that $\mathsf{Area}^{c_2^i}$ is an almost nice column with respect to $\mathsf{Area}^{c_2^{i-1}}=\mathsf{Area}^{c_1^i}$. Moreover, by Lemma \ref{lem:column}, if $c_2^i\neq c_{max}+1$, then $\mathsf{Area}^{c_2^i,c_{max}+1}>\sqrt{n}$ and $\mathsf{SCLVpointer}$ points to the first vertex of column $\mathsf{Area}^{c_2^i+1}$. So, we get that Condition \ref{lem:ColumnUpdaterCon2} is satisfied.
Observe that due to Line \ref{algo5:line15}, it follows that for every $1\leq i< k$, $c_2^i=c_1^{i+1}$; so, Condition \ref{lem:ColumnUpdaterCon3} is satisfied.
We get that $0=c_1^1<c_2^1=c_1^2<c_1^2=\ldots=c_1^k<c_2^k\leq c_{max}+1$, so $k$ is bounded. Assume that $(c_1^i,c_2^i)_{1\leq i\leq k}$ is the sequence of pairs the algorithm computes. Observe that we get that $c_2^k=c_{max}+1$, so Condition \ref{lem:ColumnUpdaterCon1} is satisfied.

Observe that the algorithm updates $\mathsf{NiceColumnsArray}$ so that for every $1\leq i\leq k$, $\mathsf{NiceColumns}$ $\mathsf{Array}[i].c_1=c_1^i$ in Lines \ref{algo5:line7} and \ref{algo5:line17},
$\mathsf{NiceColumnsArray}[i].c_2=c_2^i$ in Lines \ref{algo5:line8} and \ref{algo5:line18}, and $\mathsf{NiceColumns}$ $\mathsf{Array}[k+1].c_1=NULL$ in Line \ref{algo5:line24}. In addition, the algorithm updates $\mathsf{ColumnsArray}$ so that for every $1\leq i\leq n$, $\mathsf{ColumnsArray}[i].niceColumn=j$ where $\mathsf{NiceColumnsArray}[j].c_1<i\leq \mathsf{NiceColumnsArray}[j].c_2$ in the while loops in Lines \ref{algo5:line9} and \ref{algo5:line19}. 

Now, we prove that the algorithm runs in $\OO(n)$ time. First, by Observation \ref{lem:SCLV}, an $\mathsf{SCLV}$ of $G$ can be computed in $\OO(n)$ time. Now, observe that the total number of times Algorithm \ref{alg:NextNiceColumn} is called is $k$. For $1\leq i\leq k$, we denote the running time of the $i$-th call for Algorithm \ref{alg:NextNiceColumn} by $\mathsf{NextColumn}_i$. Observe that at the beginning of the $i$-th call for Algorithm \ref{alg:NextNiceColumn}, $\mathsf{SCLVpointer}$ points to the first vertex of the column $\mathsf{Area}^{c_1^{i}+1}$ and the algorithm returns $c_2^{i}$. Therefore, by Lemma \ref{lem:colum}, we get that the running time of the $i$-th call for Algorithm \ref{alg:NextNiceColumn} is $\OO(|\mathsf{Area}^{c_1^{i},c_2^i}|)$, so $\mathsf{NextColumn}_i=\OO(|\mathsf{Area}^{c_1^{i},c_2^i}|)$. Observe that, for every $1\leq i<j\leq k$, it follows that $\mathsf{Area}^{c_1^i,c_2^i}\cap \mathsf{Area}^{c_1^j,c_2^j}=\emptyset$, so we get that the total running time of all the calls to Algorithm \ref{alg:NextNiceColumn} is $\sum_{i=1}^k{\OO(|\mathsf{Area}^{c_1^{i},c_2^i}|)}=\OO(n)$. Similarly, we bound the total number of iterations of the while loops in Lines \ref{algo5:line9} and \ref{algo5:line19}. Observe that there are $k-1$ iterations of the while loop in Line \ref{algo5:line13}. We denote the number of iterations of the while loop in Line \ref{algo5:line9} by $\mathsf{while}_1$, and for $1\leq j\leq k-1$, we denote the number of iterations of the while loop in Line \ref{algo5:line9} during the $j$-th iteration of the while loop in Line \ref{algo5:line13} by $\mathsf{while}_{j+1}$. Observe that, for every $1\leq i\leq k$, it follows that $\mathsf{while}_i=c_2^i-c_1^i+1$. We saw that for every $1\leq i< k$, we have that $c_2^i=c_1^{i+1}$ and that $c_2^{i}<c_2^{i+1}\leq n+1$. Therefore, we get that $\sum_{i=1}^k{\mathsf{while}_i}=\OO(n)$. Notice that the running time of every such iteration is $\OO(1)$, so the total running time of the while loops in Lines \ref{algo5:line9} and \ref{algo5:line19} is $\OO(n)$. Now, observe that the rest of the computations in the while loop in Line \ref{algo5:line13} can be done in $\OO(1)$ time, and that there are $k-1\leq n$ iterations. The rest of the computations in Algorithm \ref{alg:NiceColumnsUpdater} can be done in $\OO(1)$ time. Therefore, the overall running time of Algorithm \ref{alg:NiceColumnsUpdater} is $\OO(n)$.       
\end{proof}


Our next algorithm, Algorithm \ref{alg:AreaByRowUpdater}, uses the sequence of nice columns $(c_1^i,c_2^i)_{1\leq i\leq k}$ found by Algorithm \ref{alg:NiceColumnsUpdater} to compute an $\mathsf{SRLV}$ of $\mathsf{Area}^{c_1^i,c_2^i}$, for every ${1\leq i\leq k}$, and to update $\mathsf{NiceColumnsArray}$ accordingly. After this algorithm is executed, for every ${1\leq i\leq k}$, $\mathsf{NiceColumnsArray}[i].AreaByRow$ is an $\mathsf{SRLV}$ of $\mathsf{Area}^{c_1^i,c_2^i}$. The algorithm first computes an $\mathsf{SRLV}$ of $G$. Then, the algorithm iterates over $\mathsf{SRLV}$ and adds every vertex $v_{i,j}$ to $\mathsf{NiceColumnsArray}[\mathsf{nc(j)}].AreaByRow$ where $\mathsf{nc(j)}$ is the pair $(c_1,c_2)$ of nice columns such that $c_1< j\leq c_2$.   

\begin{algorithm}[!t]
    \SetKwInOut{Input}{Input}
    \SetKwInOut{Output}{Output}
	\medskip
    {\textbf{function} $\mathsf{AreaByRowUpdater}$}$(\langle G=(V,E) \rangle)$\;
		
			$\mathsf{SRLVpointer}\gets$ $\mathsf{SRLV}$ of $G$\;
			\label{algo6:line2}\While {$\mathsf{SRLVpointer}\neq NULL$}
			{
				\label{algo6:line3}$\mathsf{currentNiceColumn}\gets \mathsf{SRLVpointer}.Column.NiceColumn$\;
				Add $\mathsf{SRLVpointer}$ to $\mathsf{currentNiceColumn}.AreaByRow$\;
				$\mathsf{SRLVpointer}\gets \mathsf{SRLVpointer}.Next$\;
			}
			
			
	
			\Return \;
				
    \caption{$\mathsf{AreaByRowUpdater}$}
    \label{alg:AreaByRowUpdater}
\end{algorithm}



In the following lemma, we prove the correctness of Algorithm \ref{alg:AreaByRowUpdater} and analyze its running time. 

\begin{lemma} \label{lem:AreaByRowUpdater}
Let $G=(V,E)$ be a connected grid graph with $n$ vertices. Let $k$ be the number of pairs $(c_1^i,c_2^i)_{1\leq i\leq k}$ found by Algorithm \ref{alg:NiceColumnsUpdater}. Then, Algorithm \ref{alg:AreaByRowUpdater} runs in $\OO(n)$ time and updates $\mathsf{NiceColumnsArray}$ as follows. For every $1\leq i\leq k$, $\mathsf{NiceColumnsArray}[i].AreaByRow$ is an $\mathsf{SRLV}$ of $\mathsf{Area}^{c_1^i,c_2^i}$.      
\end{lemma}

\begin{proof}
By Lemma \ref{lem:columnUpdater}, we get that for every $1\leq i\leq k$, $\mathsf{NiceColumnsArray}[i].c_1=c_1^i$, $\mathsf{NiceColumns}$ $\mathsf{Array}[i].c_2=c_2^i$ and $\mathsf{NiceColumnsArray}[k+1].c_1=NULL$. In addition, for every $1\leq i\leq n$, it follows that $\mathsf{ColumnsArray}[i].niceColumn=j$ where $\mathsf{NiceColumnsArray}[j].c_1<i\leq \mathsf{NiceColumns}$ $\mathsf{Array}[j].c_2$. Now, let $1\leq i\leq k$. We will show that $\mathsf{NiceColumnsArray}[i].AreaByRow$ is an $\mathsf{SRLV}$ of $\mathsf{Area}^{c_1^i,c_2^i}$. Let $u_{c,r},u_{c',r'}\in \mathsf{Area}^{c_1^i,c_2^i}$ and assume that $r<r'$. Therefore, $u_{c,r}$ appears before $u_{c',r'}$ in every $\mathsf{SRLV}$ of $G$. So, we get that the algorithm adds $u_{c,r}$ to $\mathsf{NiceColumnsArray}[i].AreaByRow$ before it adds $u_{c',r'}$ to $\mathsf{NiceColumnsArray}[i].AreaByRow$.

As for the running time, computing $\mathsf{SRLV}$ of $G$ in Line \ref{algo6:line2} can be done in $\OO(n)$ time by Observation \ref{lem:SCLV}. 
There are exactly $n$ iterations of the while loop in Line \ref{algo6:line3}, each taking $\OO(1)$ time. Therefore, we get that Algorithm \ref{alg:AreaByRowUpdater} runs in $\OO(n)$ time.    

\end{proof}


Given an $\mathsf{SRLV}$ of $\mathsf{Area}^{c_1,c_2}$ so that $c_2$ be an almost nice column with respect to $c_1$, our next algorithm (denoted Algorithm \ref{alg:AreaPrinter}) prints a sequence of nice rows between $\mathsf{Area}^{c_1}$ to $\mathsf{Area}^{c_2}$. 

\begin{algorithm}[!t]
    \SetKwInOut{Input}{Input}
    \SetKwInOut{Output}{Output}
	\medskip
    {\textbf{function} $\mathsf{AreaPrinter}$}$(\langle \mathsf{SRLVpointer},c_1,c_2 \rangle)$\;
				$r_1\gets 0$\;
		  	$r_2\gets \mathsf{NextNiceRow}\langle \mathsf{SRLVpointer}\rangle$\; 
			\label{algo7:line3}Print $\langle c_1,c_2,r_1,r_2 \rangle$\;
			\label{algo7:line4}\While {$r_2\neq r_{max}+1$}
			{
				\label{algo7:line5}$r_1\gets r_2$\;
				\label{algo7:line6}$r_2\gets \mathsf{NextNiceRow}\langle \mathsf{SCLVpointer}\rangle$\;
				\label{algo7:line7}Print $\langle c_1,c_2,r_1,r_2 \rangle$\;
			}
				\label{algo7:line8}$i\gets i+1$\;
			
			
			\Return \;
				
    \caption{$\mathsf{AreaPrinter}$}
    \label{alg:AreaPrinter}
\end{algorithm}




In the following lemma, we prove the correctness of Algorithm \ref{alg:AreaPrinter} and analyze its running time. 

\begin{lemma} \label{lem:AreaPrinter}
Let $G=(V,E)$ be a connected grid graph with $n$ vertices. Let $c_2$ be an almost nice column with respect to $c_1$. Let $\mathsf{SRLVPointer}$ be a pointer to the first vertex in an $\mathsf{SRLV}$ of $\mathsf{Area}^{c_1,c_2}$. Then, Algorithm \ref{alg:AreaPrinter} takes as input $\mathsf{SRLVPointer},c_1$ and $c_2$, runs in $\OO(|\mathsf{Area}^{c_1,c_2}|)$ time and outputs $(c_1,c_2,r_1^i,r_2^i)_{1\leq i\leq t}$ such that the following conditions are satisfied. 
\begin{enumerate}
\item $r_1^1=0$ and $r_2^t=r_{max}+1$. \label{lemAreaPCon1}
\item For every $1\leq i\leq t$, $\mathsf{Area}^{c_1,c_2}_{r_2^i}$ is an almost nice row with respect to $\mathsf{Area}^{c_1,c_2}_{r_1^i}$. \label{lemAreaPCon2}
\item For every $1\leq i< t$, $r_2^i=r_1^{i+1}$. \label{lemAreaPCon3}
\end{enumerate}
\end{lemma}

\begin{proof}
Observe that, in Line \ref{algo7:line3}, Algorithm \ref{alg:NextNiceRow} is called with $\mathsf{SRLVpointer}$ as input, where $\mathsf{SRLVpointer}$ is a pointer to the first vertex in an $\mathsf{SRLV}$ of $\mathsf{Area}^{c_1,c_2}$. Therefore, by Lemma \ref{lem:row}, Algorithm \ref{alg:NextNiceRow} returns $0<p\leq r_{max}+1$ such that $\mathsf{Area}^{c_1,c_2}_{p}$ is an almost nice row with respect to $\mathsf{Area}^{c_1,c_2}_{0}$. So, the first quadruplet the algorithm prints in Line \ref{algo7:line4} is $(c_1,c_2,0,p)$. Therefore, the sequence of quadruplets the algorithm prints is not empty. Later, we show that this sequence is finite.

Let $(c_1^i,c_2^i,r_1^i,r_2^i)_{1\leq i\leq t}$ be a prefix of the sequence of quadruplets that the algorithm prints. We show by induction that Condition \ref{lemAreaPCon2} is satisfied for every $1\leq i\leq t$. We argue that for every $1\leq i\leq t$, it follows that $\mathsf{Area}^{c_1,c_2}_{r_2^i}$ is an almost nice row with respect to $\mathsf{Area}^{c_1,c_2}_{r_1^i}$. Moreover, if $r_2^i\neq r_{max}+1$, then $\mathsf{Area}^{c_1,c_2}_{r_2^i,r_{max}+1}>\sqrt{n}$ and $\mathsf{SRLVpointer}$ points to the first vertex of row $\mathsf{Area}^{c_1,c_2}_{r_2^i+1}$ at the time that the algorithm prints $(c_1^i,c_2^i,r_1^i,r_2^i)$. 

For $i=1$, we saw that Condition \ref{lemAreaPCon2} is satisfied. Now, if in Line \ref{algo7:line4} Algorithm \ref{alg:NextNiceRow} returns $r_2\neq r_{max}+1$, then by Lemma \ref{lem:row}, we get that $\mathsf{Area}^{c_1,c_2}_{r_2^i,r_{max}+1}>\sqrt{n}$ and $\mathsf{SRLVpointer}$ points to the first vertex of row $\mathsf{Area}^{c_1,c_2}_{r_2^i+1}$. Observe that $\mathsf{SRLVpointer}$ does not change by the time the algorithm prints $(c_1^1,c_2^1,r_1^1,r_2^1)$, thus we have proved the statement for $i=1$.

Now, let $1< i\leq t$. Observe that the algorithm prints $(c_1^i,c_2^i,r_1^i,r_2^i)$ in Line \ref{algo7:line8}. Therefore, because of the condition of the while loop in Line \ref{algo7:line5}, we get that $r_2^{i-1}\neq n+1$. Therefore, by the inductive hypothesis, we get that $\mathsf{Area}^{c_1,c_2}_{r_2^{i-1},r_{max}+1}>\sqrt{n}$ and $\mathsf{SRLVpointer}$ points to the first vertex of row $\mathsf{Area}^{c_1,c_2}_{r_2^{i-1}+1}$. Therefore, by Lemma \ref{lem:row}, we get that in Line \ref{algo7:line7} Algorithm \ref{alg:NextNiceRow} returns $r_2^{i-1}<r_2^i\leq r_{max}+1$ such that $\mathsf{Area}^{c_1,c_2}_{r_2^i}$ is an almost nice row with respect to $\mathsf{Area}^{c_1,c_2}_{r_2^{i-1}}=\mathsf{Area}^{c_1,c_2}_{r_1^{i}}$. Moreover, by Lemma \ref{lem:row}, if $r_2^i\neq r_{max}+1$ then $\mathsf{Area}^{c_1,c_2}_{r_2^i,r_{max}+1}>\sqrt{n}$ and $\mathsf{SRLVpointer}$ points to the first vertex of row $\mathsf{Area}^{c_1,c_2}_{r_2^i+1}$. So, we get that Condition \ref{lemAreaPCon2} is satisfied.

Observe that, due to Line \ref{algo7:line6}, it follows that for every $1\leq i< t$, $r_2^i=r_1^{i+1}$; therefore, Condition \ref{lemAreaPCon3} is satisfied.

Therefore, we get that $0=r_1^1<r_2^1=r_1^2<r_1^2=\ldots=r_1^t<r_2^t\leq r_{max}+1$, so $t$ is bounded. Assume that $(c_1^i,c_2^i,r_1^i,r_2^i)_{1\leq i\leq t}$ is the sequence of quadruplets the algorithm prints. Observe that, $r_2^t=r_{max}+1$, so Condition \ref{lemAreaPCon1} is satisfied.

Now, we show that the algorithm runs in time $\OO(|\mathsf{Area}^{c_1,c_2}|)$. Observe that the total number of times the algorithm calls Algorithm \ref{alg:NextNiceRow} is $t$. For $1\leq i\leq t$, we denote the running time of the $i$-th call for Algorithm \ref{alg:NextNiceRow} by $\mathsf{NextRow}_i$. Observe that, at the beginning of the $i$-th call for Algorithm \ref{alg:NextNiceRow}, $\mathsf{SRLVpointer}$ points to the first vertex in row $\mathsf{Area}^{c_1,c_2}_{r_1^i+1}$ and the algorithm returns $r_2^{i}$. Therefore, by Lemma \ref{lem:row}, we get that the running time of the $i$-th call for Algorithm \ref{alg:NextNiceColumn} is $\OO(|\mathsf{Area}^{c_1,c_2}_{r_1^i,r_2^i}|)$, so $\mathsf{NextRow}_i=\OO(|\mathsf{Area}^{c_1,c_2}_{r_1^i,r_2^i}|)$. Observe that, for every $1\leq i<j\leq t$, it follows that $\mathsf{Area}^{c_1,c_2}_{r_1^i,r_2^i}\cap \mathsf{Area}^{c_1,c_2}_{r_1^j,r_2^j}=\emptyset$, so we get that the total running time of all the calls for Algorithm \ref{alg:NextNiceRow} is $\sum_{i=1}^t{\OO(|\mathsf{Area}^{c_1,c_2}_{r_1^i,r_2^i}|)}=\OO(|\mathsf{Area}^{c_1,c_2}|)$.   
                   


\end{proof}





%\begin{lemma} \label{lem:algoNiceC}
%Let $G=(V,E)$ be a grid graph and let $H=(V',E')$ be the good super rectangle grid graph of $G$. Let $\mathsf{SCLVpointer}$  be a pointer to the first vertex of a column $\mathsf{Area}^{c_i}$ of $G$ in the SCLV of $G$. If $\mathsf{Area}^{c_i,n}>\sqrt{n}$ then Algorithm \ref{alg:NextNiceColumn} returns $c_j$ such that $\mathsf{Area}^{c_j}$ is an almost nice column with respect to $\mathsf{Area}^{c_i}$. Moreover, if $c_j< n+1$ then $\mathsf{Area}^{c_j,n+1}>\sqrt{n}$.
%\end{lemma}

%\begin{proof}
%Notice that Algorithm \ref{alg:NextNiceColumn} counts every vertex by the order of the columns. First, at step \ref{algo3:while1} it finds a column $\mathsf{Area}^{c_j}$, such that $\mathsf{Area}^{c_i,c_j}>\sqrt{n}$. Then, notice that at step \ref{algo3:while2} it finds the minimum $c_\ell \geq c_j$ such that $\mathsf{Area}^{c_\ell}\leq \sqrt{n}$. Therefore, if there exists a nice column with respect to $\mathsf{Area}^{c_i}$, then $\mathsf{Area}^{c_\ell}$ is such a column. Now, notice that because $\mathsf{Area}^{c_i,n}>\sqrt{n}$, we know that such a column exists, due to Lemma \ref{lem:Nice column}. Now, notice that at step \ref{algo3:while3} the algorithm checks if $\mathsf{Area}^{c_j,n}>\sqrt{n}$. If $\mathsf{Area}^{c_j,n}>\sqrt{n}$, it returns $c_j$, and the conditions of the lemma stand. Otherwise, it returns $n+1$. In that case, by definition, $\mathsf{Area}^{n+1}$ is an almost nice column with respect to $\mathsf{Area}^{c_i}$. Therefore, in any case the conditions of the lemma stand.   
%\end{proof}

%\begin{lemma} \label{lem:algoNiceR}
%Let $G=(V,E)$ be a grid graph and let $H=(V',E')$ be the good super rectangle grid graph of $G$. Let $c_1,c_2$ be two natural numbers such that $\mathsf{Area}^{c_1}$ is an almost nice column with respect to $\mathsf{Area}^{c_2}$. Let $0\leq r\leq n+1$. Let $\mathsf{SCLVpointer}$ be a pointer to the first vertex of row  $\mathsf{Area}^{c_1,c_2}_{r}$ in the SCLV of $G$. Let $\mathsf{SRLVpointer}$  be a pointer to the first vertex of row $\mathsf{Area}^{c_1,c_2}_{r}$ of $G$ in the SRLV of $G$. If $\mathsf{Area}^{c_1,c_2}_{r,n+1}>\sqrt{n}$ then Algorithm \ref{alg:NextNiceRow} returns $r'$ such that $\mathsf{Area}^{c_1,c_2}_{r'}$ is a nice row with respect to $\mathsf{Area}^{c_1,c_2}_{r}$. Moreover, if $r'< n+1$ then $\mathsf{Area}^{c_1,c_2}_{r',n+1}>\sqrt{n}>\sqrt{n}$. At the end of the algorithm, $\mathsf{SCLVpointer}$ and $\mathsf{SRLVpointer}$  point at the first vertex of row $\mathsf{Area}^{c_1,c_2}_{r'}$, or at the first vertex of $\mathsf{Area}^{c_2}$ if $r'=n+1$.  
%\end{lemma}

%\begin{proof}
%Notice that at step \ref{algo2while1} that Algorithm \ref{alg:NextNiceRow} counts every vertex by the order of the row between the two columns $\mathsf{Area}^{c_1}$
%and $\mathsf{Area}^{c_2}$. First, it finds the minimum $r'' \geq r$ such that $\mathsf{Area}^{c_1,c_2}_{r,r''}\geq \sqrt{n}$. Therefore, if there exists a nice row with respect to $\mathsf{Area}^{c_1,c_2}_{r}$, $\mathsf{Area}^{c_1,c_2}_{r''}$ is such a row. Now, notice that because $\mathsf{Area}^{c_1,c_2}_{r,n+1}>\sqrt{n}$, we know that such a row exists, due to Lemma \ref{lem:nice row}. Now, if $\mathsf{Area}^{c_1,c_2}_{r'',n+1}< \sqrt{n}$ then the algorithm returns $n+1$. In that case $\mathsf{Area}^{c_1,c_2}_{n+1}$ is a nice row with respect to $\mathsf{Area}^{c_1,c_2}_{r}$. Notice that the pointers at the end of the algorithm points at the right vertices according to the lemma, because of steps \ref{pointers}.  
%\end{proof}


%\begin{lemma}
%Let $G=(V,E)$ be a grid graph. Then Algorithm \ref{alg:PrintGraphDecomposition} prints a sequence of quadruplets $(c_1^i,c_2^i,r_1^i,r_2^i)_{1\leq i\leq k}$ such that, the sequence is a nice RCL-cover.
%\end{lemma}

%\begin{proof}
%Let $(c_1^i,c_2^i,r_1^i,r_2^i)_{1\leq i\leq k}$ be the sequence quadruplets the Algorithm \ref{alg:PrintGraphDecomposition} prints for $G=(V,E)$. 
%First we show that for every $1\leq i\leq k$ it follows that $\mathsf{Area}^{c_2^i}$ is an almost nice column with respect to $\mathsf{Area}^{c_1^i}$, and $\mathsf{Area}^{c_1^i,c_2^i}_{r_2^i}$ is a nice row with respect to $\mathsf{Area}^{c_1^i,c_2^i}_{r_1^i}$. As for the first quadruplets, $c_1^1=0$, and because $|\mathsf{Area}^{0,n+1}|=|V(G)|>\sqrt(n)$, and $\mathsf{SRLVpointer}$ points to the first vertex in $\mathsf{Area}^{0}$, then by Lemma \ref{lem:algoNiceC} Algorithm \ref{alg:NextNiceColumn} returns $c_2^1$ such that $\mathsf{Area}^{c_2^1}$ is an almost nice column with respect to $\mathsf{Area}^{0}$. Now, because $\mathsf{Area}^{c_2^1}$ is an almost nice column with respect to $\mathsf{Area}^{0}$, and $r_1^1=0$, it follows that $|\mathsf{Area}^{0,c_2^1}_{0,n+1}|=|\mathsf{Area}^{0,c_2^1}|\geq \sqrt{n}$. Now because $\mathsf{SRLVpointer}$ and $\mathsf{SRLVpointer}$ point to the first vertex of row $\mathsf{Area}^{0,c_1^2}_0$ at the beginning of the algorithm, then by Lemma \ref{lem:algoNiceR}, Algorithm \ref{alg:NextNiceRow} returns $r_2^1$ such that $\mathsf{Area}^{0,c_2^1}_{r_2^1}$ is a nice row with respect to $\mathsf{Area}^{0,c_2^1}_{0}$. Now, we want to show that this condition stands also for every quadruplet that was printed during step \ref{Algo4step8}. Notice that if $r_2^1=n+1$ then no quadruplet was printed during that step. Suppose that $r_2^1\neq n+1$. Notice that for every quadruplet $j$ that was printed during that step, it follows that $c_1^j=c_1^1$ and $c_2^j=c_2^1$, therefore $\mathsf{Area}^{c_2^j}$ is an almost nice column with respect to $\mathsf{Area}^{c_1^j}$. Now, let $i$ be an arbitrary quadruplet $i$ that was printed during that step. Because for the previous quadruplet, $r_2^{i-1}\neq n+1$, by Lemma \ref{lem:algoNiceR} we know that $|\mathsf{Area}^{c_1^j,c_2^j}_{r_2^{i-1},n+1}|\geq \sqrt{n}$. Therefore, by using \ref{lem:algoNiceR} again, we know that Algorithm \ref{alg:NextNiceRow} returns $r_2^i$ such that $\mathsf{Area}^{c_1^i,c_2^i}_{r_2^i}$ is a nice row with respect to $\mathsf{Area}^{c_1^i,c_2^i}_{r_2^{i-1}}$. Observe that can use same arguments to show that this condition stands also for every quadruplet that was printed during step \ref{Algo4step16}. Therefore, for every $1\leq i\leq k$ it follows that $\mathsf{Area}^{c_2^i}$ is an almost nice column with respect to $\mathsf{Area}^{c_1^i}$, and $\mathsf{Area}^{c_1^i,c_2^i}_{r_2^i}$ is a nice row with respect to $\mathsf{Area}^{c_1^i,c_2^i}_{r_1^i}$.

%Now, we aim to show that $(c_1^i,c_2^i,r_1^i,r_2^i)_{1\leq i\leq k}$ is an RCL-Cover. For that purpose, we show that the conditions of Definition \ref{def:RCL} stand. As for the first condition, because we saw that for every $1\leq i\leq k$ it follows that $\mathsf{Area}^{c_2^i}$ is an almost nice column with respect to $\mathsf{Area}^{c_1^i}$, and $\mathsf{Area}^{c_1^i,c_2^i}_{r_2^i}$ is a nice row with respect to $\mathsf{Area}^{c_1^i,c_2^i}_{r_1^i}$, by Definition \ref{def:Nice column} and Definition \ref{def:Nice Row} we know that $c_2^i>c_1^i$ and $r_2^i>r_1^i$ for every $1\leq i\leq k$.

%Now we want to show that the second condition stands. Observe that if for $1\leq i,j\leq k$ it follows that $c_1^i=c_1^j$, then both of the quadruplets $i$ and $j$ were printed at step \ref{Algo4step8}, or at the same loop of the second while \ref{algo4:2ndWhile}. Therefore, it follows that $c_2^i=c_2^j$. Now, looking at an arbitrary loop of the second while \ref{algo4:2ndWhile}. Assume that quadruplets $i$ to $j$ were printed during that loop. Observe that for each $1\leq i\leq \ell <j\leq k$ it follows that $r_1^\ell=r_2^{\ell -1}$, and we saw that also $r_1^\ell \leq r_2^{\ell}$. Therefore we get that $(r_1^i, r_2^i, r_1^{i+1}, r_2^{i+1} \ldots r_1^j,r_2^j)$ is an increase sequence. A similar arguments can prove that it holds for quadruplets that were printed at earlier steps.

%Similarly, if $c_1^i=c_1^j$ then the quadruplets $i$ and $j$  were not printed at the same loop of the second while \ref{algo4:2ndWhile}. Now, let $i_0=1$ and $i_1,\ldots, i_\ell \in \{1,\ldots, k\}$ be the first quadruplets that were printed at any first loop of the inner loop \label{algo4:3rdWhile}. Then for each $0\leq m< \ell$ it follows that $c_1^{i_m}=c_2^{i_{m-1}}$. Consider that we saw that $c_1^i \leq c_2^i$, we get that $(c_1^{i_0}, c_2^{i_0}, c_1^{i_1}, c_2^{i_1} \ldots c_1^{i_\ell},c_2^{i_\ell}$ is an increase sequence. Observe that $c_1^{i_0}=0$, and $c_2^{i_\ell}=n+1$, and that proves the third condition of Definition \ref{def:RCL}. Now, using same arguments for quadruplets that were printed at earlier steps, we can say that the sequence $(c_1^1, c_2^1, c_1^{2}, c_2^{2} \ldots c_1^k,c_2^k)$ is an increase sequence, and that completes the proof of the second condition.

%Now we want to show that the last condition stands. Let $1\leq \ell \leq k$. let $1\leq i\leq \ell \leq j k$  be the first and last quadruplets that were printed during the same loop of the the second while \ref{algo4:2ndWhile} that the $i$-th quadruplet was printed. Observe that for any $i\leq m<j$ it follows that $r_2^i=r_1^{i+1}$. Consider that we saw that $r_1^m \leq r_2^m$. Moreover, by the conditions of the algorithm $r_1^i=0$ and $r_2^j=n+1$. Now, using same arguments for quadruplets that were printed at earlier steps, we see that the last condition stands.

%Therefore, the sequence of quadruplets $(c_1^i,c_2^i,r_1^i,r_2^i)_{1\leq i\leq k}$ that the Algorithm \ref{alg:PrintGraphDecomposition} prints is an RCL-Cover. We also saw that for every $1\leq i\leq k$ it follows that $\mathsf{Area}^{c_2^i}$ is an almost nice column with respect to $\mathsf{Area}^{c_1^i}$, and $\mathsf{Area}^{c_1^i,c_2^i}_{r_2^i}$ is a nice row with respect to $\mathsf{Area}^{c_1^i,c_2^i}_{r_1^i}$. Then, by using to Lemma \ref{lem:niceRCL}, we get that $(c_1^i,c_2^i,r_1^i,r_2^i)_{1\leq i\leq k}$ is a nice RCL-Cover.                         
    
%%We need to show that the conditions of Definition \ref{def:RCL} stand. As for the first condition. For $(c_1^1,c_2^1,r_1^1,r_2^1)$, observe that $c_1^1=0$, and by Lemma \ref{lem:algoNiceC}, $c_2^1$ is an almost nice column with respect to $c_1^1$, therefore by Definition \ref{def:Nice column} it follows that $c_1^1\leq c_2^1$. Now, notice that every quadruplet that the algorithm prints in the step \ref{Algo4step6}, has the same $c_1$ and $c_2$ as the first quadruplet, so the first condition is valid to these quadruplets as well.             
%\end{proof}

%\begin{algorithm}
 %   \SetKwInOut{Input}{Input}
  %  \SetKwInOut{Output}{Output}
	%\medskip
   % {\textbf{function} $\mathsf{NextNiceRow}$}$(\langle \mathsf{SCLVpointer}, \mathsf{SRLVpointer}, c_1, c_2, r \rangle)$\;
		
    %	 $\mathsf{Area}\gets 0$ \;
		
			% $\mathsf{CurrentRow}\gets \mathsf{SRLVpointer.row}$ \;
			%\label{algo2while1}
			%\While{$\mathsf{Area}< \sqrt{n}$   }{$\mathsf{Area} \gets \mathsf{Area}+1$ \; $\mathsf{SRLVpointer}\gets \mathsf{SRLVpointer.Next}$ \; \If {$\mathsf{SRLVpointer.column}>c_2$ Or $\mathsf{SRLVpointer.column}<c_1$} {\While{$\mathsf{SCLVpointer.row}\leq \mathsf{CurrentRow}$}{$\mathsf{SCLVpointer}\gets \mathsf{SCLVpointer.Next}$}    $\mathsf{SRLVpointer}\gets \mathsf{SCLVpointer}$\; $\mathsf{CurrentRow}\gets \mathsf{SRLVpointer.row}$ \;}}
			%\While{$\mathsf{SCLVpointer.row}\leq \mathsf{CurrentRow}$ And $\mathsf{SCLVpointer.row}\leq c_2 $}{$\mathsf{SCLVpointer}\gets \mathsf{SCLVpointer.Next}$\; \label{pointer} } $\mathsf{SRLVpointer}\gets \mathsf{SCLVpointer}$\;
			%$\mathsf{RestOfArea}\gets 0$\;
			%$\mathsf{SRLVpointerTemp}\gets \mathsf{SRLVpointer}$ \;
			%$\mathsf{SCLVpointerTemp}\gets \mathsf{SCLVpointer}$ \;
			%\While{$\mathsf{RestOfArea}< \sqrt{n}$ And $\mathsf{SCLVpointerTemp.column\leq c_2}$}{$\mathsf{RestOfArea} \gets \mathsf{RestOfArea}+1$ \; $\mathsf{SRLVpointerTemp}\gets \mathsf{SRLVpointerTemp.Next}$\;
			%\If {$\mathsf{SRLVpointerTemp.column}>c_2$ Or $\mathsf{SRLVpointerTemp.column}<c_1$}  
			%{\While{$\mathsf{SCLVpointerTemp.row}\leq \mathsf{CurrentRowTemp}$}{$\mathsf{SCLVpointerTemp}\gets \mathsf{SCLVpointerTemp.Next}$}    $\mathsf{SRLVpointerTemp}\gets \mathsf{SCLVpointerTemp}$\;}
			
		%	}
			%\If {$\mathsf{RestOfArea}<\sqrt{n}$} {\Return $n+1$} \Else {\Return $\mathsf{CurrentRow}$} 
			
	
    %\caption{$\mathsf{NextNiceRow}$}
    %\label{alg:NextNiceRow}
%\end{algorithm}








%\begin{algorithm}
 %   \SetKwInOut{Input}{Input}
  %  \SetKwInOut{Output}{Output}
	%\medskip
   % {\textbf{function} $\mathsf{PrintGraphDecomposition}$}$(\langle \mathsf{SCLVpointer}, \mathsf{SRLVpointer} \rangle)$\;
		
    %	$c_1\gets 0$\;
			%$c_2\gets \mathsf{NextNiceColumn}\langle \mathsf{SCLVpointer}, \mathsf{SRLVpointer} \rangle$ \;
			%$r\gets \mathsf{NextNiceRow}\langle \mathsf{SCLVpointer}, \mathsf{SRLVpointer}, c_1, c_2, 0 \rangle$ \; 
			%Print $\langle c_1,c_2,r \rangle$ \;
			%\While {$r\neq n+1$}
			%{
			%	$r\gets \mathsf{NextNiceRow}\langle \mathsf{SCLVpointer}, \mathsf{SRLVpointer}, c_1, c_2, r \rangle$ \; 
			%	Print $\langle c_1,c_2,r \rangle$ \; \label{Algo4step8}
			%}
			%\label{algo4:2ndWhile}
			%\While {$c_2 \neq n+1$} 
			%{
			%$c_1\gets c_2$\;
			%$c_2\gets \mathsf{NextNiceColumn}\langle \mathsf{SCLVpointer}, \mathsf{SRLVpointer} \rangle$ \; 
		%	$r\gets 0$ \;
		%	\label{algo4:3rdWhile}
		%	\While {$r\neq n+1$} 
		%	{
		%		$r\gets \mathsf{NextNiceRow}\langle \mathsf{SCLVpointer}, \mathsf{SRLVpointer}, c_1, c_2, r \rangle$ \; 
		%		Print $\langle c_1,c_2,r \rangle$ \; \label{Algo4step16}
		%	}
			
		%	}
			%\Return \;
				
    %\caption{$\mathsf{PrintGraphDecomposition}$}
    %\label{alg:PrintGraphDecomposition}
%\end{algorithm}

Finally, we are ready to present Algorithm \ref{alg:PrintGraphDecomposition}, which employs (directly or indirectly) the algorithms we have seen so far in order to compute a nice RCL-cover of $G$. 
First, we find nice columns using Algorithm \ref{alg:NiceColumnsUpdater}. Then, we compute the $\mathsf{SRLV}$ of each rectangle $\mathsf{Area}_{c_1^i,c_2^i}$ found by using Algorithm \ref{alg:AreaByRowUpdater}. Finally, we use Algorithm \ref{alg:AreaPrinter} in order to print the nice rows in each rectangle $\mathsf{Area}_{c_1^i,c_2^i}$.   


\begin{algorithm}[!t]
    \SetKwInOut{Input}{Input}
    \SetKwInOut{Output}{Output}
	\medskip
    {\textbf{function} $\mathsf{PrintGraphDecomposition}$}$(\langle G=(V,E) \rangle)$\;
			$\mathsf{NiceColumnsUpdater}(G)$\;
			\label{algo8:line2}$\mathsf{AreaByRowUpdater}(G)$\;
		\label{algo8:line3}	$i\gets 1$\;
			\While{$\mathsf{NiceColumnsArray}[i].c_1\neq Null$}
			{
				\label{algo8:line5}$c_1\gets \mathsf{NiceColumnsArray}[i].c_1$\;
				$c_2\gets \mathsf{NiceColumnsArray}[i].c_2$\;
				$\mathsf{SRLVpointer}\gets \mathsf{NiceColumnsArray}[i].AreaByRow$\; 
				$\mathsf{AreaPrinter}(\langle \mathsf{SRLVpointer},c_1,c_2 \rangle)$\;
				$i\gets i+1$\;
			}
			
			\Return \;
				
    \caption{$\mathsf{PrintGraphDecomposition}$}
    \label{alg:PrintGraphDecomposition}
\end{algorithm}



In the next lemma, we prove the correctness of Algorithm \ref{alg:PrintGraphDecomposition} by invoking Lemma \ref{lem:niceRCL}, and analyze its running time. 

\begin{lemma} \label{lem:column}
Let $G=(V,E)$ be a connected grid graph with $n$ vertices. Then, Algorithm \ref{alg:PrintGraphDecomposition} takes $G=(V,E)$ as input, runs in time $\OO(n)$, and prints a nice RCL-cover of $G$. 
\end{lemma}

%{def:niceDe} 
%Let $G=(V,E)$ be a connected grid graph. A {\em nice decomposition} of $G$ is a sequence of subsets of $V$ $(U_i)_{1\leq i\leq k}$ such that the following conditions are satisfied.
%\begin{enumerate}
%\item For every $v\in V(G)$, there exists $1\leq i\leq k$ such that $v\in U_i$. \label{dcon1}

\begin{proof}
We first show that Algorithm \ref{alg:PrintGraphDecomposition} prints an RCL-cover of $H$. Notice that in Line \ref{algo8:line2} the algorithm calls Algorithm \ref{alg:NiceColumnsUpdater} with $G$ as input. Therefore, by Lemma \ref{lem:columnUpdater}, there exist $(c_1^i,c_2^i)_{1\leq i\leq \ell}$ such that $c_1^1=0, c_2^k=c_{max}+1$, $c_2^i$ is an almost nice column with respect to $c_2^i$ and $c_2^i=c_1^{i+1}$ for every $1\leq i<\ell$. Moreover, $1\leq i\leq k$ $\mathsf{NiceColumnsArray}[i].c_1=c_1^i$, $\mathsf{NiceColumnsArray}[i].c_2=c_2^i$ and $\mathsf{NiceColumnsArray}[\ell+1].c_1=NULL$. Now, in Line \ref{algo8:line3}, the algorithm calls Algorithm \ref{alg:AreaByRowUpdater} with $G$ as input . Therefore, by Lemma \ref{lem:AreaByRowUpdater}, for every $1\leq i\leq \ell$, $\mathsf{ColumnsArray}[i].AreaByRow$ is an $\mathsf{SRLV}$ of $\mathsf{Area}^{c_1^i,c_2^i}$. We get that $\mathsf{NiceColumnsArray}[1].c_1\neq NULL$, so by Lemma \ref{lem:AreaPrinter}, the algorithm prints $(c_1^1,c_2^1,r_1^i,r_2^i)_{1\leq i\leq t_1}$. So, the sequence of quadruplets that the algorithm prints is not empty. Later, we show that this sequence is finite.  

Let $(c_1^i,c_2^i,r_1^i,r_2^i)_{1\leq i\leq k}$ be a prefix of the sequence of quadruplets the algorithm prints. First, we show that Condition \ref{def:RCL Con1} of Definition \ref{def:RCL} is satisfied, that is for every $1\leq i\leq k$, $c^i_2>c_1^i$ and $r^i_2>r_1^i$. In addition, we show that for every $1\leq i\leq k$, $\mathsf{Area}^{c_2^i}$ is an almost nice column with respect to $\mathsf{Area}^{c_2^i}$, and $\mathsf{Area}^{c_2^i,c_2^i}_{r_2^i}$ is an almost nice row with respect to $\mathsf{Area}^{c_2^i,c_2^i}_{r_1^i}$. We have already seen that, for $i=1$, these claims are satisfied.

Let $1\leq j\leq k$. Let $1\leq i\leq \ell$ be the iteration of the while loop in Line \ref{algo8:line5} where the algorithm prints $(c_1^j,c_2^j,r_1^j,r_2^j)$. By Lemma \ref{lem:AreaByRowUpdater}, we get that $\mathsf{ColumnsArray}[i].AreaByRow$ is an $\mathsf{SRLV}$ of $\mathsf{Area}^{c_1^j,c_2^j}$, and by Lemma \ref{lem:columnUpdater}, we get that $\mathsf{Area}^{c_2^j}$ is an almost nice column with respect to $\mathsf{Area}^{c_1^j}$, therefore $c_2^j>c_1^j$. By Lemma \ref{lem:AreaPrinter}, we get that $\mathsf{Area}^{c_2^i,c_2^i}_{r_2^i}$ is an almost nice row with respect to $\mathsf{Area}^{c_2^i,c_2^i}_{r_1^i}$, therefore $r^i_2>r_1^i$.

%That is, we show that for every $1\leq i\leq \ell$, the condition is satisfied for every quadruplet $(c_1^j,c_2^j,r_1^j,r_2^j)$ that was printed until the $i$-th iteration.
Now, we prove that Condition \ref{def:RCL Con2} of Definition \ref{def:RCL} is satisfied, that is, for every $1\leq i<j\leq k$: if $c_1^i=c_1^j$, then $c_2^i=c_2^j$ and $r_1^j\geq r_2^i$; otherwise, $c_1^j\geq c_2^i$. We show this by induction on the iteration number $\ell$. For $\ell=1$, let $(c_1^1,c_2^1,r_1^i,r_2^i)_{1\leq i\leq t_1}$ be the quadruplets the algorithm prints in the first iteration. Let $1\leq i<j\leq t_1$. Since $(c_1^i,c_2^i,r_1^i,r_2^i)$ and $(c_1^j,c_2^j,r_1^j,r_2^j)$ are printed in the same iteration, they are printed by a call of Algorithm \ref{alg:AreaPrinter}. Therefore, by Lemma \ref{lem:AreaPrinter}, we get that $c_1^i=c_1^j$ and $c_2^i=c_2^j$. We show by induction on $t_1$ that $r_1^j\geq r_2^i$. The base case $t_1=1$ is trivial. For $t_1=s>1$, if  $1\leq i<j< s$, then by the inductive hypothesis we get that $r_1^j\geq r_2^i$. If $1\leq i<j= s$, then by Lemma \ref{lem:AreaByRowUpdater}, we get that $r_1^s=r_2^{s-1}$, so if $i=s-1$ we are done. Otherwise, from Lemma \ref{lem:AreaByRowUpdater}, we get that $r_1^s=r_2^{s-1}>r_1^{s-1}$, and by the inductive hypothesis, we get that $r_1^{s-1}\geq r_2^{j}$, so $r_1^s=r_2^{s-1}>r_1^{s-1}\geq r_2^{j}$. 
For $\ell=d>1$, if $(c_1^i,c_2^i,r_1^i,r_2^i)$ and $(c_1^j,c_2^j,r_1^j,r_2^j)$ are both not printed in the $d$-th iteration, then by the inductive hypothesis we get that if $c_1^i=c_1^j$ then $c_2^i=c_2^j$ and $r_1^j\geq r_2^i$. Assume that $(c_1^j,c_2^j,r_1^j,r_2^j)$ is printed in the $d$-th iteration and $(c_1^i,c_2^i,r_1^i,r_2^i)$ is printed in the $d'$-th iteration for $1\leq d'<d$. If $d'=d-1$, then by Lemma \ref{lem:columnUpdater} we get that $c_1^d=c_2^{d-1}>c_1^{d-1}$, and we are done. Otherwise, by Lemma \ref{lem:columnUpdater} we get that $c_2^{d-1}>c_1^{d-1}$, and from the inductive hypothesis we get that $c_1^{d-1}\geq c_2^{d'}$, so $c_1^d=c_2^{d-1}>c_1^{d-1}\geq c_2^{d'}>c_1^{d'}$. The case where $d=d'$ can be proved similarly.

Now, we show that Condition \ref{def:RCL Con3} of Definition \ref{def:RCL} is satisfied, that is, there exist $1\leq i_1<i_2<\ldots<i_\ell \leq k$ such that $c_1^{i_1}=0$, $c_2^{i_\ell}=c_{max}+1$ and for every $1\leq j<\ell$, $c_1^{i_{j+1}}=c_2^{i_{j}}$. For every $1\leq j\leq \ell$, let $i_j$ be such that $(c_1^{i_j},c_2^{i_j},r_1^{i_j},r_2^{i_j})$ is the first quadruplet that the algorithm prints in the $j$-th iteration of the while loop in Line \ref{algo8:line5}. Observe that $c_1^{i_j}=c^j_1$ and $c_2^{i_j}=c^j_2$ where $(c^j_1,c^j_2)_{1\leq j\leq \ell}$ are the pairs that Algorithm \ref{alg:NiceColumnsUpdater} finds in Line \ref{algo8:line2}. Therefore, by Lemma \ref{lem:columnUpdater}, we get that $c_1^1=c_1^{i_1}=0$, $c_2^\ell=c_2^{i_\ell}=c_{max}+1$, and for every $1\leq j< \ell$, $c_1^{i_{j+1}}=c_1^{j+1}=c_2^{j}=c_2^{i_{j}}$.

Lastly, we show that Condition \ref{def:RCL Con4} of Definition \ref{def:RCL} is satisfied, that is, for every $1\leq i\leq k$ there exist $s\leq i\leq t$ such that $c_1^s=c_1^t=c_1^i, r_1^s=0$ and $r_2^t=r_{max}+1$, and for every $s\leq m<t$, $r_1^{m+1}=r_2^m$. Let $1\leq i\leq k$. Let $1\leq j\leq \ell$ be the iteration in the while loop in Line \ref{algo8:line5} where the algorithm prints $(c_1^{i},c_2^{i},r_1^{i},r_2^{i})$. Let $s\leq i\leq t$ be such that $(c_1^{s},c_2^{s},r_1^{s},r_2^{s})$ and $(c_1^{t},c_2^{t},r_1^{t},r_2^{t})$ are the first and last quadruplets, respectively, that the algorithm prints in the $j$-th iteration. Then, by Lemma \ref{lem:AreaByRowUpdater}, we get that $c_1^s=c_1^t=c_1^i, r_1^s=0$ and $r_2^t=r_{max}+1$, and for every $s\leq m<t$, $r_1^{m+1}=r_2^m$. 

We have shown that all the conditions of Definition \ref{def:RCL} are satisfied, therefore $(c_1^i,c_2^i,r_1^i,r_2^i)_{1\leq i\leq k}$ is an RCL-cover of $H$. In addition, we saw that for every $1\leq i\leq k$ it follows that $\mathsf{Area}^{c_2^i}$ is an almost nice column with respect to $\mathsf{Area}^{c_2^i}$ and $\mathsf{Area}^{c_2^i,c_2^i}_{r_2^i}$ is an almost nice row with respect to $\mathsf{Area}^{c_2^i,c_2^i}_{r_1^i}$. Therefore, by Lemma \ref{lem:niceRCL}, we get that the algorithm prints a nice RCL-cover of $G$.

Now, we show that the running time of the algorithm is $\OO(n)$. First, the calls to Algorithms \ref{alg:NiceColumnsUpdater} and \ref{alg:AreaByRowUpdater} in Lines \ref{algo8:line2} and \ref{algo8:line3} take $\OO(n)$ running time by Lemmas \ref{lem:columnUpdater} and \ref{lem:AreaByRowUpdater}. Now, observe that the total numbers of times the algorithm calls Algorithm \ref{alg:AreaPrinter} is $k$. For $1\leq i\leq k$, we denote the running time of the $i$-th call to Algorithm \ref{alg:AreaPrinter} by $\mathsf{AreaPrinter}_i$. Observe that, at the beginning of the $i$-th call to Algorithm \ref{alg:AreaPrinter}, $\mathsf{SRLVpointer}$ is a pointer to the $\mathsf{SRLV}$ of $\mathsf{Area}^{c_1^i,c_2^i}$. Therefore, by Lemma \ref{lem:AreaPrinter}, we get that the running time of the $i$-th call to Algorithm \ref{alg:AreaPrinter} is $\OO(|\mathsf{Area}^{c_1^i,c_2^i}|)$, so $\mathsf{AreaPrinter}_i=\OO(|\mathsf{Area}^{c_1^i,c_2^i}|)$. Observe that, for every $1\leq i<j\leq k$, it follows that $\mathsf{Area}^{c_1^i,c_2^i}\cap \mathsf{Area}^{c_1^j,c_2^j}=\emptyset$, so we get that the total running time of all the calls to Algorithm \ref{alg:AreaPrinter} is $\sum_{i=1}^k{\OO(|\mathsf{Area}^{c_1^i,c_2^i}|)}=\OO(n)$. The rest of the computations of the algorithm take $\OO(1)$ time. The number of iterations of the while loop in Line \ref{algo8:line5} is $k\leq n$. Therefore, we get that the total running time of the algorithm is $\OO(n)$.                                      
\end{proof}



In Lemma \ref{lem:column}, we have shown the existence of an algorithm that finds a nice RCL-cover in $\OO(n)$ time. This, in turn, concludes the proof of Theorem \ref{lem:algo exists}.

Observe that we can easily adapt the algorithm to return also the sets corresponding to a nice RCL-cover $(c_1^i,c_2^i,r_1^i,r_2^i)_{1\leq i\leq k}$ of $G$, $(\mathsf{Area}^{c_1^i,c_2^i}_{r_1^i,r_2^i})_{1\leq i\leq k}$, in the same running time (bound by $\OO(n)$). The change we need to do is in Algorithm \ref{alg:NextNiceRow}, where we find the ``next nice row". In addition to counting the vertices, we can also put the vertices in a set, and return this set in addition to the next nice row.    

%\begin{lemma} \label{lem:column2}
%Let $G=(V,E)$ be a connected grid graph with $n$ vertices. Then Algorithm \ref{alg:PrintGraphDecomposition} with the input $G=(V,E)$ works in time $\OO(n)$ and prints a nice RCL-cover of $G$. 
%\end{lemma}

%\begin{proof}
%We show that Algorithm \ref{alg:PrintGraphDecomposition} prints a nice RCL-cover of $G$. Notice that in Line 3 Algorithm \ref{alg:NextNiceColumn} is given the input $\mathsf{SCLVpointer}$, where $\mathsf{SCLVpointer}$ is a pointer to the first vertex in the $\mathsf{SCLVpointer}$ of $G$. Therefore, by Lemma \ref{lem:colum}Algorithm \ref{alg:NextNiceColumn} returns $0<j\leq n+1$ such that $\mathsf{Area}^{j}$ is an almost nice column with respect to $\mathsf{Area}^{0}$. Similarly, in Line 6 Algorithm \ref{alg:NextNiceRow} is given the input $\mathsf{SRLVpointer}$, where $\mathsf{SRLVpointer}$ is a pointer to the first vertex in the $\mathsf{SRLVpointer}$ of $\mathsf{Area}^{i,j}$. Therefore, by Lemma \ref{lem:row} Algorithm \ref{alg:NextNiceRow} returns $0<p\leq n+1$ such that $\mathsf{Area}^{0,j}_{p}$ is a nice row with respect to $\mathsf{Area}^{0,j}_{p}$. So the first quadruplet the algorithm prints is $(0,j,0,p)$. Therefore the sequence of quadruplets the algorithm prints is not empty. Later we show that this sequence is finite.

%Let $(c_1^i,c_2^i,r_1^i,r_2^i)_{1\leq i\leq k}$ be an affix of the sequence of quadruplets the algorithm prints. First we show that Condition 1 of Definition 3.8 is satisfied, that is for every $1\leq i\leq k$ it follows that $c^i_2>c_1^i$ and $r^i_2>r_1^i$. In addition, we show that for every $1\leq i\leq k$ it follows that $\mathsf{Area}^{c_2^i}$ is an almost nice column with respect to $\mathsf{Area}^{c_2^i}$ and $\mathsf{Area}^{c_2^i,c_2^i}_{r_2^i}$ is a nice row with respect to $\mathsf{Area}^{c_2^i,c_2^i}_{r_1^i}$. We saw that for $i=1$ the claims are satisfied.

%Now we show that these claims are satisfied for every quadruplet that the algorithm prints in Line 11. Assume that $(c_1^i,c_2^i,r_1^i,r_2^i)_{2\leq i\leq m}$ are the quadruplets the algorithm prints in Line 11 for some $2\leq m\leq k-1$. Denote the $\mathsf{SRLVpointer}$ at the beginning of the $i$-th iterations of the while loop in Line 8, where $(c_1^{i+1},c_2^{i+1},r_1^{i+1},r_2^{i+1})$ is printed in Line 11, by $\mathsf{SRLVpointer}_{i+1}$. We show by induction that for every $2\leq i\leq m-1$ it follows that $c^i_2>c_1^i$, $r^i_2>r_1^i$, $\mathsf{Area}^{c_2^i}$ is an almost nice column with respect to $\mathsf{Area}^{c_2^i}$, $\mathsf{Area}^{c_2^i,c_2^i}_{r_2^i}$ is a nice row with respect to $\mathsf{Area}^{c_2^i,c_2^i}_{r_1^i}$ and $\mathsf{SRLVpointer}_{i}$ points to the first vertex in row $\mathsf{Area}^{c_2^i,c_2^i}_{r_2^i+1}$. Observe that for every $2\leq i\leq m$ it follows that $c_1^i=c_1^1, c_2^i=c_2^2$, so we get that $c^i_2>c_1^i$ and $\mathsf{Area}^{c_2^i}$ is an almost nice column with respect to $\mathsf{Area}^{c_2^i}$. For $i=2$, observe that $r_2^1\neq n+1$, otherwise the condition of the while loop in Line 8 was not satisfied. Therefore, by Lemma \ref{lem:row}, we get that $\mathsf{SRLVpointer}_{2}$ points to the first vertex in row $\mathsf{Area}^{c_2^1,c_2^1}_{r_1^1+1}$ and $\mathsf{Area}^{c_2^1,c_2^1}_{r_2^1,n+1}\geq \sqrt{n}$. Therefore, by Lemma \ref{lem:row} in Line 10 Algorithm \ref{alg:NextNiceRow} returns $r_2^2$ such that $\mathsf{Area}^{c_2^2,c_2^2}_{r_2^2}$ is a nice row with respect to $\mathsf{Area}^{c_2^2,c_2^2}_{r_1^2}$, and therefore also $r_2^2>r_1^2$. Since $2<m$ it follows that $r_2^2\neq n+1$, otherwise the condition of the while loop in Line 8 was not satisfied. Therefore, by Lemma \ref{lem:row}, we get that $\mathsf{SRLVpointer}_{3}$ points to the first vertex in row $\mathsf{Area}^{c_2^2,c_2^2}_{r_2^2+1}$ and $\mathsf{Area}^{c_1^2,c_2^2}_{r_2^2,n+1}\geq \sqrt{n}$. The proof for the inductive step can be shown similarly. The proof for case $i=m$ can be shown similarly, using that $\mathsf{SRLVpointer}_{m}$ points to the first vertex in row $\mathsf{Area}^{c_2^{m-1},c_2^{m-1}}_{r_2^{m-1}+1}$ and $\mathsf{Area}^{c_1^{m-1},c_2^{m-1}}_{r_2^{m-1},n+1}\geq \sqrt{n}$.

%Now, observe that $(c_1^i,c_2^i,r_1^i,r_2^i)_{m+1\leq i\leq k}$ are printed inside the while loop in Line 13. Let $\ell$ be the number of iterations in this loop. Observe that for every $1\leq i\leq \ell$ there exist $c_1^i, c_2^i$ such that every quadruplet $(c_1^j,c_2^j,r_1^j,r_2^j)$ that is printed in the $i$-th iteration, it follows that $c_1^j=c_1^i$ and $c_2^j=c_2^i$. We denote the $\mathsf{SCLVpointer}$ at the beginning of the $i$-th iteration by $\mathsf{SCLVpointer}_{i}$. We show by induction, that for every $1\leq i\leq \ell-1$, the claims for the quadruplets that the algorithm prints in the $i$-th iteration are satisfied and also $\mathsf{SCLVpointer}_{i}$ points to the first vertex in column $\mathsf{Area}^{c_2^i}$ at the end of the iteration. For $i=1$, observe that $c_2^{m}\neq n-1$, otherwise the condition of the while loop in Line 13 was not satisfied. Therefore, by Lemma \ref{lem:colum} it follows that $\mathsf{SCLVpointer}_1$ which is the $\mathsf{SCLVpointer}$ that the Algorithm \ref{alg:NextNiceColumn} returns, points to the first vertex in column $\mathsf{Area}^{c_2^m+1}$ and $\mathsf{Area}^{c_2,n+1}\geq \sqrt{n}$. Therefore, by Lemma \ref{lem:colum} it follows that Algorithm \ref{alg:NextNiceColumn} in Line 15 returns a $c_2(1)$ such that $\mathsf{Area}^{c_2(1)}$ is an almost nice column with respect to $\mathsf{Area}^{c_1(1)}$ and so $c_2(1)>c_1(1)$. Moreover, since $1<\ell$ we get that $c_2(1)<n+1$, therefore, be Lemma \ref{lem:colum} it follows that the $\mathsf{SCLVpointer}$ in Line 15 points to the first vertex in column $\mathsf{Area}^{c_2(1)+1}$ and $\mathsf{Area}^{c_2(1),n+1}\geq \sqrt{n}$. Observe that the $\mathsf{SRLVpointer}$ in Line 16 points to the first vertex in row $\mathsf{Area}^{c_1(1),c_2(1)}_{0}$ and also $\mathsf{Area}^{c_1(1),c_2(1)}_{0,n+1}\geq \sqrt{n}$. Therefore, by Lemma \ref{lem:row}, Algorithm \ref{alg:NextNiceRow} returns $r_2^{m+1}$ such that $\mathsf{Area}^{c_1(1),c_2(1)}_{r_2^{m+1}}$ is a nice row with respect to $\mathsf{Area}^{c_1(1),c_2(1)}_{0}$and so $r_2^{m+1}>0$. Therefore, the claims for the quadruplet $(c_1^{m+1},c_2^{m+1},r_1^{m+1},r_2^{m+1})$ that is printed in Line 19 are satisfied. The proof for the quadruplets that are printed in Line 22 can be shown similarly to the proof of the quadruplets that are printed in Line 11. The proof for the inductive step can be shown similarly. The proof for case $i=\ell$ can be shown similarly, using that $\mathsf{SCLVpointer}_{\ell-1}$ points to the first vertex in column $\mathsf{Area}^{c_2({\ell-1})+1}$ and $\mathsf{Area}^{c_2({\ell-1}),n+1}\geq \sqrt{n}$. This ends the proof for these claims.

%Now we show that assume that the number of quadruplets the algorithm prints is finite. Assume that $(c_1^i,c_2^i,r_1^i,r_2^i)_{2\leq i\leq m}$ are printed in the while loop in Line 8. Observe that for each $2\leq i<m$ it follows that $r_2^i=r_2^{i+1}$. Therefore, combining the claims we proved, it follows that $r_2^2<r_2^3<\ldots<r_2^m$ and since $r_2^m\leq n+1$, it follows that the $m\geq n+1$ and therefore the number of quadruplets the algorithm prints inside this while loop is finite. It can be proved similarly that the number of quadruplets the algorithm prints inside this while loop is finite. 

%Now we show that Condition 3 of the RCL-cover is satisfied. We need to show that there exists $1\leq i_1<i_2<\ldots<i_\ell\leq k$ such that $c_1^{i_1}=0$, $c_2^{i_\ell}=n+1$ and for every $1\leq j<\ell$ it follows that $c_1^{i_{j+1}}=c_1^{i_{j+1}}$. Let $t$ be the number of iterations of the while loop in Line 13. Let                                        
%\end{proof}

\section{Path Decomposition}

In this section, we show that given a nice RCL-cover of a grid graph $G$, we can compute a path decomposition of $G$ of width $\OO(\sqrt{n})$ in $\OO(n)$ time, where each bag corresponds to a rectangle (and the columns that ``flank'' it). We have the main theorem of this section:

\begin{theorem}\label{th:pathdec}
There exists an algorithm that given a connected grid graph $G$, a nice RCL-cover of $G$, $(c_1^i,c_2^i,r_1^i,r_2^i)_{1\leq i\leq k}$ and the corresponding sets, $(\mathsf{Area}^{c_1^i,c_2^i}_{r_1^i,r_2^i})_{1\leq i\leq k}$, computes a path decomposition of $G$ of width $\OO(\sqrt{n})$ in $\OO(n)$ time. 
\end{theorem}

We begin with our construction of a path decomposition. Given a nice RCL-cover of $G$, $(c_1^i,c_2^i,r_1^i,r_2^i)_{1\leq i\leq k}$ and the corresponding sets, $(\mathsf{Area}^{c_1^i,c_2^i}_{r_1^i,r_2^i})_{1\leq i\leq k}$, we construct a path with $k$ vertices, that is, ${\cal P}=(V_P,E_P)$ where $V_P=\{v_1,\ldots,v_k\}$ and $E_P=\{\{v_i,v_{i+1}\}~|~1\leq i\leq k-1\}$. We assign to every ``bag" $v_i$ the set of vertices in the corresponding rectangle $(c_1^i,c_2^i,r_1^i,r_2^i)$, that is, the set of vertices $\mathsf{Area}^{c_1^i,c_2^i}_{r_1^i,r_2^i}$, the vertices in the $c_1^i$-th and the $c_2^i$-th columns of $G$ (that is, $\mathsf{Area}^{c_1^i}$ and $\mathsf{Area}^{c_2^i}$), and the vertices in row $\mathsf{Area}^{c_1^i,c_2^i}_{r_1^i}$ (see Figures \ref{fi:pathdecoEx} and \ref{fi:pathdecoEx2}). We show that this construction is a path decomposition of $G$ of width $\OO(\sqrt{n})$ in the next lemma:


\begin{figure}[t!]
\centering
\includegraphics[width=0.75\textwidth, page=5]{figures/fig.pdf}
\caption{Example of a bag of our path decomposition construction, corresponding to the rectangle in orange, in the given nice RCL-cover of $G$. The vertices included in this ``bag" are the vertices in the orange rectangle, $\mathsf{Area}_{6,8}^{13,19}$, the vertices of the $13$-th and $19$-th columns (marked in red), and the vertices of row $\mathsf{Area}^{13,19}_{6}$ (marked in red). Observe that the vertices of row $\mathsf{Area}^{13,19}_{8}$ are contained in $\mathsf{Area}_{6,8}^{13,19}$ (and are also marked in red).}\label{fi:pathdecoEx}
\end{figure}


\begin{figure}[t!]
\centering
\includegraphics[width=0.75\textwidth, page=6]{figures/fig.pdf}
\caption{Example of the construction of our path decomposition, corresponding to the nice RCL-cover of $G$, that is illustrated in the figure. The path decomposition is written at the bottom of the figure.}\label{fi:pathdecoEx2}
\end{figure}

 %Observe that, since $(c_1^i,c_2^i,r_1^i,r_2^i)_{1\leq i\leq k}$ is a nice RCL-cover of $G$, then $|\mathsf{Area}^{c_1^i,c_2^i}_{r_1^i,r_2^i}|=\OO(\sqrt{n})$. In addition, since $\mathsf{Area}^{c_1^i}$ and $\mathsf{Area}^{c_2^i}$ are almost nice columns, and $\mathsf{Area}^{c_1^i,c_2^i}_{r_1^i}$ and $\mathsf{Area}^{c_1^i,c_2^i}_{r_2^i}$ are almost nice rows, then $|\mathsf{Area}^{c_1^i}|=\OO(\sqrt{n})$, $|\mathsf{Area}^{c_2^i}|=\OO(\sqrt{n})$, $|\mathsf{Area}^{c_1^i,c_2^i}_{r_1^i}|=\OO(\sqrt{n})$ and $|\mathsf{Area}^{c_1^i,c_2^i}_{r_2^i}|=\OO(\sqrt{n})$. Therefore, each ``bag" is assign to a subset of $V$ of size $\OO(\sqrt{n})$

\begin{lemma}\label{lem:pathDec}
Let $G$ be a grid graph, let $(c_1^i,c_2^i,r_1^i,r_2^i)_{1\leq i\leq k}$ be a nice RCL-cover of $G$ and let $(\mathsf{Area}^{c_1^i,c_2^i}_{r_1^i,r_2^i})_{1\leq i\leq k}$ be the corresponding sets. Let ${\cal P}=(V_P,E_P)$ where $V_P=\{v_1,\ldots,v_k\}$ and $E_P=\{\{v_i,v_{i+1}\}~|~1\leq i\leq k-1\}$. Let $\beta: V_P\rightarrow 2^V$, where $\beta(v_i)=\mathsf{Area}^{c_1^i,c_2^i}_{r_1^i,r_2^i}\cup \mathsf{Area}^{c_1^i}\cup \mathsf{Area}^{c_2^i}\cup \mathsf{Area}^{c_1^i,c_2^i}_{r_1^i}$ for all $v_i\in V_P$. Then, $({\cal P},\beta)$ is a path decomposition of $G$ of width $\OO(\sqrt{n})$.    
\end{lemma}   

\begin{proof}
First we show that $({\cal P},\beta)$ is a path decomposition of $G$. We need to show that the conditions of Definition \ref{def:pathDeco} are satisfied. Let $u\in V$. Since $(c_1^i,c_2^i,r_1^i,r_2^i)_{1\leq i\leq k}$ is a nice RCL-cover of $G$, there must be ${1\leq i\leq k}$ such that $u\in \mathsf{Area}^{c_1^i,c_2^i}_{r_1^i,r_2^i}$. If $u\in \mathsf{Area}^{c_1^i,c_2^i}_{r_1^i,r_2^i}\setminus (\mathsf{Area}^{c_1^i,c_2^i}_{r_2^i}\cup \mathsf{Area}^{c_2^i})$, then $\{ v\in V_P~|~u\in \beta(v)\}=\{v_i\}$, so Condition \ref{def:pathDecocon1} is satisfied. Otherwise, $u\in \mathsf{Area}^{c_1^i,c_2^i}_{r_2^i}\cup \mathsf{Area}^{c_2^i}$. Assume that $u\in \mathsf{Area}^{c_2^i}$. Let $m\leq i\leq \ell$ be the minimal and maximal indexes such that $c_2^i=c_2^m=c_2^\ell$. Since $(c_1^i,c_2^i,r_1^i,r_2^i)_{1\leq i\leq k}$ is a nice RCL-cover of $G$, we get that for every $m\leq i'\leq \ell$, $c_2^{i'}=c_2^i$. Now, by Definition \ref{def:RCL}, we get that $c_1^{\ell+1}=c_2^i$. Let $\ell+1\leq s$ be the maximal index such that $c_1^{\ell+1}=c_1^s$. Since $(c_1^i,c_2^i,r_1^i,r_2^i)_{1\leq i\leq k}$ is a nice RCL-cover of $G$, we get that for every $\ell+1 \leq i'\leq s$, $c_1^{i'}=c_1^{\ell+1}$. Therefore, we get that for every $m \leq i'\leq s$, $u\in \beta(i')$. Now, again, since $(c_1^i,c_2^i,r_1^i,r_2^i)_{1\leq i\leq k}$ is a nice RCL-cover of $G$, for every $i'<m$, $c_2^{i'}<c_2^i$, so $u\notin \beta(i')$, and for every $i'>m$, $c_1^{i'}>c_2^i$, so $u\notin \beta(i')$. Therefore, we get that $\{ v\in V_P~|~u\in \beta(v)\}=\{v_m,v_{m+1},\ldots v_{s-1},v_s\}$, so Condition \ref{def:pathDecocon1} is satisfied. Now, assume that $u\in \mathsf{Area}^{c_1^i,c_2^i}_{r_2^i}\setminus \mathsf{Area}^{c_2^i}$. Observe that $\mathsf{Area}^{c_1^i,c_2^i}_{r_2^i}=\mathsf{Area}^{c_1^{i+1},c_2^{i+1}}_{r_1^{i+1}}$, so we get that $v\in \beta(v_i)\cap \beta(v_{i+1})$. Notice that for every $i'<i$ and $i'>i+1$, $v\notin \beta(v_{i+1})$. Therefore, we get that $\{ v\in V_P~|~u\in \beta(v)\}=\{v_i,v_{i+1}\}$, so Condition \ref{def:pathDecocon1} is satisfied. We get that at any case, Condition \ref{def:pathDecocon1} is satisfied. 

We now aim to show that Condition \ref{def:pathDecocon2} is satisfied. Let $\{u,v\}\in E$. Since $(c_1^i,c_2^i,r_1^i,r_2^i)$ is a nice RCL-cover of $G$, there must be ${1\leq i\leq k}$ such that $u\in \mathsf{Area}^{c_1^i,c_2^i}_{r_1^i,r_2^i}$. Now, if $v\in \mathsf{Area}^{c_1^i,c_2^i}_{r_1^i,r_2^i}$, then $u,v\in \mathsf{Area}^{c_1^i,c_2^i}_{r_1^i,r_2^i}\subseteq \beta(v_i)$, and so, Condition \ref{def:pathDecocon2} is satisfied. Otherwise, $u\notin \mathsf{Area}^{c_1^i,c_2^i}_{r_1^i,r_2^i}$ so $v\in B(\mathsf{Area}^{c_1^i,c_2^i}_{r_1^i,r_2^i})$. If $u\in \mathsf{Area}^{c_1^i}\cup \mathsf{Area}^{c_1^i,c_2^i}_{r_1^i}$, then $u,v\in \mathsf{Area}^{c_1^i,c_2^i}_{r_1^i,r_2^i}\cup \mathsf{Area}^{c_1^i}\cup \mathsf{Area}^{c_1^i,c_2^i}_{r_1^i}\cup \subseteq \beta(v_i)$, and so, Condition is satisfied. Otherwise, $v\in \mathsf{Area}^{c_2^i}\cup \mathsf{Area}^{c_1^i,c_2^i}_{r_2^i}$. In this case, if $v\in \mathsf{Area}^{c_1^i,c_2^i}_{r_2^i}$, then $u\in \mathsf{Area}^{c_1^i,c_2^i}_{r_2^i+1}\subseteq \mathsf{Area}^{c_1^{i+1},c_2^{i+1}}_{r_1^{i+1},r_2^{i+1}}\subseteq \beta(v_{i+1})$. Now, observe that $v\in \mathsf{Area}^{c_1^i,c_2^i}_{r_2^i}=\mathsf{Area}^{c_1^{i+1},c_2^{i+1}}_{r_1^{i+1}}\subseteq \beta(v_{i+1})$. Therefore, we get that $u,v\in \beta(v_{i+1})$. The case where $v\in \mathsf{Area}^{c_2^i}$ is similar. So, Condition \ref{def:pathDecocon2} is satisfied. Thus, $({\cal P},\beta)$ is a path decomposition of $G$.   
 
Now, for every $1\leq i\leq k$, since $(c_1^i,c_2^i,r_1^i,r_2^i)_{1\leq i\leq k}$ is a nice RCL-cover of $G$, then $|\mathsf{Area}^{c_1^i,c_2^i}_{r_1^i,r_2^i}|=\OO(\sqrt{n})$. In addition, $\mathsf{Area}^{c_1^i}$ and $\mathsf{Area}^{c_2^i}$ are almost nice columns, and $\mathsf{Area}^{c_1^i,c_2^i}_{r_1^i}$ is almost nice row, so $|\mathsf{Area}^{c_1^i}|=\OO(\sqrt{n})$, $|\mathsf{Area}^{c_2^i}|=\OO(\sqrt{n})$ and $|\mathsf{Area}^{c_1^i,c_2^i}_{r_1^i}|=\OO(\sqrt{n})$. Therefore, we get that $|\beta(v_i)|=\OO(\sqrt{n})$. Thus, we have proved that $(P,\beta)$ is a path decomposition of $G$ of width $\OO(\sqrt{n})$.  
\end{proof}       


Now, we present an algorithm that given a nice RCL-cover of $G$, $(c_1^i,c_2^i,r_1^i,r_2^i)_{1\leq i\leq k}$, and the corresponding sets, $(\mathsf{Area}^{c_1^i,c_2^i}_{r_1^i,r_2^i})_{1\leq i\leq k}$, computes $(\beta(v_i))_{1\leq i\leq k}$, as defined in Lemma \ref{lem:pathDec}, in $\OO(n)$ time. 

In the next lemma, we prove the correctness of Algorithm \ref{alg:RCL-CoverToPathDecomposition} and analyze its running time:


\begin{lemma} \label{pathdecoalg}
Let $G$ be a connected grid graph, let $(c_1^i,c_2^i,r_1^i,r_2^i)_{1\leq i\leq k}$ be a nice RCL-cover of $G$ and let $(\mathsf{Area}^{c_1^i,c_2^i}_{r_1^i,r_2^i})_{1\leq i\leq k}$ be the corresponding sets. Then Algorithm \ref{alg:RCL-CoverToPathDecomposition} takes $(c_1^i,c_2^i,r_1^i,r_2^i)_{1\leq i\leq k}$ and $(\mathsf{Area}^{c_1^i,c_2^i}_{r_1^i,r_2^i})_{1\leq i\leq k}$ as input, and returns $(\beta(v_i))_{1\leq i\leq k}$ such that, for every $1\leq i\leq k$, $\beta(v_i)$=$\mathsf{Area}^{c_1^i,c_2^i}_{r_1^i,r_2^i}\cup \mathsf{Area}^{c_1^i}\cup \mathsf{Area}^{c_2^i}\cup \mathsf{Area}^{c_1^i,c_2^i}_{r_1^i}$. Moreover, Algorithm \ref{alg:RCL-CoverToPathDecomposition} runs in $\OO(n)$ time.     
\end{lemma}    

\begin{proof}
Observe that after Line \ref{alg10:line1}, we get that for every $1\leq i\leq n$, $C(i)=\mathsf{Area}^i$. Therefore, after Line \ref{alg10:line2}, we get that for every $1\leq i\leq k$, $\beta(v_i)=\mathsf{Area}^{c_1^i,c_2^i}_{r_1^i,r_2^i}\cup \mathsf{Area}^{c_1^i}\cup \mathsf{Area}^{c_2^i}$. Now, we show that for every $1\leq i\leq k-1$, $\mathsf{Area}^{c_1^{i+1},c_2^{i+1}}_{r_1^{i+1}}=\mathsf{Area}^{c_1^i,c_2^i}_{r_2^i}$. Observe that if $r_1^{i+1}\neq 0$, then $\mathsf{Area}^{c_1^{i+1},c_2^{i+1}}_{r_1^{i+1}}=\mathsf{Area}^{c_1^i,c_2^i}_{r_2^i}$. Otherwise, $r_1^{i+1}=0$, so $\mathsf{Area}^{c_1^{i+1},c_2^{i+1}}_{r_1^{i+1}}=\emptyset$, and $r_2^{i}=n+1$, so $\mathsf{Area}^{c_1^i,c_2^i}_{r_2^i}=\emptyset$; therefore, $\mathsf{Area}^{c_1^{i+1},c_2^{i+1}}_{r_1^{i+1}}=\mathsf{Area}^{c_1^i,c_2^i}_{r_2^i}$. Now, notice that after Line \ref{alg10:line3}, $R(2)=\mathsf{Area}^{c_1^i,c_2^i}_{r_2^i}=\mathsf{Area}^{c_1^{i+1},c_2^{i+1}}_{r_1^{i+1}}$. Therefore, after Line \ref{alg10:line4}, $\beta(v_i)$=$\mathsf{Area}^{c_1^i,c_2^i}_{r_1^i,r_2^i}\cup \mathsf{Area}^{c_1^i}\cup \mathsf{Area}^{c_2^i}\cup \mathsf{Area}^{c_1^i,c_2^i}_{r_1^i}$, for every $2\leq i\leq k$. As for $\beta(v_1)$, observe that $\mathsf{Area}^{c_1^1,c_2^1}_{r_1^1}=\emptyset$, so $\beta(v_1)$=$\mathsf{Area}^{c_1^1,c_2^1}_{r_1^1,r_2^1}\cup \mathsf{Area}^{c_1^1}\cup \mathsf{Area}^{c_2^1}\cup \mathsf{Area}^{c_1^1,c_2^1}_{r_1^1}$. Thus, we have proved the correctness of the algorithm.

As for the running time, the computations in Lines \ref{alg10:line0} and \ref{alg10:line-1} take $\OO(n)$ time. The computations in Lines \ref{alg10:line7} and \ref{alg10:line8} take $\OO(n)$ time as well. Observe that in the for loop in Line \ref{alg10:line220} every vertex in $V$ is considered only once, therefore the total running time of this for loop is $\OO(n)$. The rest of the computations take $\OO(1)$ time. Thus, the total running time of the algorithm is $\OO(n)$.          

\end{proof}

\begin{algorithm}[!t]
    \SetKwInOut{Input}{Input}
    \SetKwInOut{Output}{Output}
	\medskip
    {\textbf{function} $\mathsf{RCL-CoverToPathDecomposition}$}$(\langle (c_1^i,c_2^i,r_1^i,r_2^i)_{1\leq i\leq k}, (\mathsf{Area}^{c_1^i,c_2^i}_{r_1^i,r_2^i})_{1\leq i\leq k} \rangle)$\;
		Create $n$ empty sets $C(i)$ for every $1\leq i\leq n$\;
		\label{alg10:line-1}
		\For {every $u_{i,j}\in V$}
		{
			\label{alg10:line0}
		$C(j)\gets C(j)\cup \{u_{i,j}\}$\;
		}
		\label{alg10:line1}
		Create $k$ empty sets $\beta(v_i)$ for every $1\leq i\leq k$\;
		\label{alg10:line7}
		\For {every $1\leq i\leq k$}
	{\label{alg10:line8}
		$\beta(v_i)\gets \mathsf{Area}^{c_1^i,c_2^i}_{r_1^i,r_2^i}\cup C(c_1^i)\cup C(c_2^i)$\;
		}
		\label{alg10:line2}
		\For {every $1\leq i\leq k-1$}
		{
		Create an empty list $R(2)$\;
	\For {every $u_{\ell,j}\in \mathsf{Area}^{c_1^i,c_2^i}_{r_1^i,r_2^i}$}
	{
	\label{alg10:line220}
	\If{$\ell= r_2^i$}
	{
	$R(2)\gets R(2)\cup u_{\ell,j}$\;  
	}
	}
	\label{alg10:line3}
	$\beta(v_{i+1})\gets \beta(v_{i+1})\cup R(2)$\; 
	$R(2)\gets \emptyset$\;
		}
		\label{alg10:line4}
		\Return $(\beta(v_i))_{1\leq i\leq k}$\;
	
				
    \caption{$\mathsf{RCL-CoverToPathDecomposition}$}
    \label{alg:RCL-CoverToPathDecomposition}
\end{algorithm}


In Lemma \ref{lem:pathDec}, we have proved the correctness of our construction of a path decomposition of $G$, and in Lemma \ref{pathdecoalg} we have shown the existence of an algorithm that computes this construction in $\OO(n)$ time. This, in turn, concludes the proof of Theorem \ref{th:pathdec}.



==> makefile <==
finalname = main

included_latex_sources = 
compiler = pdflatex
psfiles = \


$(finalname): $(included_latex_sources) $(psfiles) $(finalname).tex
	$(compiler) $(finalname).tex

%.ps: %.fig
	fig2dev -Leps $< $@

%.ps: %.gif
	convert $< $@

%.ps: %.bmp
	convert $< $@

%.ps: %.jpg
	convert $< $@

startup:
	xemacs $(finalname).tex &
	xdvi $(finalname) &
	xfig -bg white -fg black &

clean:
	rm -f $(psfiles)
	rm -f $(finalname).ps
	rm -f tmp-data/*.avg
	rm -f tmp-data/*.txt
	rm -f src-data/*.tmp
	rm -f *~
	rm -f *.bak
	rm -f figures/*.bak
	rm -f *.toc
	rm -f *.aux
	rm -f *.blg
	rm -f *.dvi
	rm -f *.log
	rm -f *.bbl 
	rm -f *.idx 
	rm -f *.out 
	# rm -f $(finalname).pdf
	rm -f *.thm
	rm -f *synctex
	rm -f *synctex.gz
	rm -f *.sav
	rm -f *.vtc
	rm -f *.fdb_latexmk
	rm -f *.fls
	rm -f *.brf

bib: 
	$(compiler) $(finalname).tex
	bibtex $(finalname)
	bibtex appendix
	$(compiler) $(finalname).tex
	$(compiler) $(finalname).tex



ps: $(finalname)
	dvips -t a4 $(finalname).dvi -o # -pp 6 -t a4

#	dvips -t letter $(finalname).dvi -o

pdf: 
	$(compiler) $(finalname).tex

level: 
	$(compiler) mainLevel.tex
	
clique: 
	$(compiler) mainClique.tex	
	
print: ps
	lpr -Ppolaris -h $(finalname).ps


